Towards Reliable Test-Time Adaptation: Style Invariance as a Correctness Likelihood

Test-time adaptation (TTA) enables efficient adaptation of deployed models, yet it often leads to poorly calibrated predictive uncertainty - a critical issue in high-stakes domains such as autonomous driving, finance, and healthcare. Existing calibration methods typically assume fixed models or static distributions, resulting in degraded performance under real-world, dynamic test conditions. To address these challenges, we introduce Style Invariance as a Correctness Likelihood (SICL), a framework that leverages style-invariance for robust uncertainty estimation. SICL estimates instance-wise correctness likelihood by measuring prediction consistency across style-altered variants, requiring only the model's forward pass. This makes it a plug-and-play, backpropagation-free calibration module compatible with any TTA method. Comprehensive evaluations across four baselines, five TTA methods, and two realistic scenarios with three model architecture demonstrate that SICL reduces calibration error by an average of 13 percentage points compared to conventional calibration approaches.

==> figs/ablation.tex <==
\begin{figure*}[t!]
%\begin{figure*}[H]
    \centering
    \includegraphics[width=\linewidth]{wacv-2026-author-kit-template/figs/raw_figs/ablation_final.pdf}
    \caption{Ablation results on (a) individual components of SICL, (b) relaxation term - gain in expected calibration error via relaxation term, and (c) performances upon the number of variants $N$ across baseline TTA algorithms.}
    \label{fig:ablation_studies}
    \vspace{-10pt}
\end{figure*}

==> figs/backgrounds.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figs/raw_figs/backgrounds.pdf} % Set to \columnwidth to fit within one column
    \caption{Conceptual demonstration of content-driven predictions with style (\textit{e.g.} texture) and content (\textit{e.g.} shape) differentiation.}
    % caption{Demonstration of content-driven predictions by a trained model with style (\textit{e.g.} texture) and content (\textit{e.g.} shape) differentiation.}
    \label{Fig:backgrounds}
    \vspace{-10pt}
\end{figure}



==> figs/observation.tex <==
\begin{figure*}[t!]
%\begin{figure*}[H]
    \centering
    \includegraphics[width=\linewidth]{wacv-2026-author-kit-template/figs/raw_figs/observation.png}
    \caption{
    Observations upon TTA calibration patterns: (a) \& (b) show reliability and calibration error changes across temporal distribution shifts, while (c) \& (d) display these changes under a fixed Gaussian Noise corruption.
    }
    \label{Fig:observation}
    \vspace{-10pt}
\end{figure*}

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/2_related_work.tex <==

\definecolor{lightcyan}{RGB}{224, 240, 255} % Light cyan color for rows
\definecolor{headercyan}{RGB}{200, 220, 240} % Slightly darker cyan for header
\definecolor{verylightblue}{RGB}{235, 245, 255} % Very light blue for "o"
\definecolor{verylightred}{RGB}{255, 235, 235} % Very light red for "x"
\newcommand{\cmark}{\checkmark} % Checkmark symbol
\newcommand{\xmark}{\textbf{\texttimes}} % Bold "x" symbol
\section{Related Work}\label{sec:related_work}


\paragraph{Uncertainty Calibration.} 
The goal of calibration is to align the confidence of a model with its actual accuracy, ensuring that the probability estimates reflect the true predictive uncertainty. Existing methods~\cite{guo2017calibration, liu2022devil, ding2021local, balanya2024adaptive, yu2022robust} typically exploit temperature scaling to adjust the logit. \textit{Temperature-scaling methods} assume a fixed model and distribution, scaling the entire data with a single temperature. As a result, they fail to address the varying characteristics of each test instance under various distribution changes and changing models. Moreover, obtaining the temperature often requires additional training with labeled data~\cite{guo2017calibration, wang2020transferable, park2020calibrated}, or pseudo-data~\cite{hupseudo}, which are unavailable at test time and adds a burden on top of the adaptation process. Meanwhile, \textit{ensembling methods} ~\cite{gal2016dropout, lakshminarayanan2017simple} use dropout or model ensembling by averaging stochastic predictions (ensemble candidates) for more reliable confidence estimates. However, dropout often produces poor candidate representations due to its process of randomly disabling neurons of the model (Section \ref{sec:motivation}). Also, Deep Ensembles~\cite{lakshminarayanan2017simple} require training several models, which is undesirable in TTA. As illustrated in Table \ref{tab:calibration_comparison}, existing methods face several limitations when applied to TTA setup, underscoring the need for tailored calibration strategies for real-world TTA.
%\noindent\textbf{Test-Time Adaptation.} 




%\begin{table}[htbp]
% \begin{table}[t!]
%     \centering
%     \tiny % Reduce font size
%     \renewcommand{\arraystretch}{1} % Adjust row height for readability
%     \setlength{\tabcolsep}{2pt} % Adjust column spacing
%     \resizebox{\columnwidth}{!}{  
%     \begin{tabular}{>{\centering\arraybackslash}p{1.5cm} |>{\centering\arraybackslash}p{1cm} >{\centering\arraybackslash}p{1cm} >{\centering\arraybackslash}p{1cm} >{\centering\arraybackslash}p{1cm}}
%         \toprule
%         Calibration Method & No Source Data & No Extra Training & No Harm to Accuracy & Instance-wise Calibration \\
%         \midrule
%         Vanilla TS~\cite{guo2017calibration} & \cellcolor{verylightred}$\xmark$ & \cellcolor{verylightred}$\xmark$ & \cellcolor{verylightblue}$\cmark$ & \cellcolor{verylightred}$\xmark$ \\
%         MC Dropout~\cite{gal2016dropout} & \cellcolor{verylightblue}$\cmark$ & \cellcolor{verylightblue}$\cmark$ & \cellcolor{verylightred}$\xmark$ & \cellcolor{verylightblue}$\cmark$ \\
%         TransCal~\cite{wang2020transferable} & \cellcolor{verylightred}$\xmark$ & \cellcolor{verylightred}$\xmark$ & \cellcolor{verylightblue}$\cmark$ & \cellcolor{verylightred}$\xmark$ \\
%         PseudoCal~\cite{hupseudo}  & \cellcolor{verylightblue}$\cmark$ & \cellcolor{verylightred}$\xmark$ & \cellcolor{verylightblue}$\cmark$ & \cellcolor{verylightred}$\xmark$ \\
%         SICL(Ours) & \cellcolor{verylightblue}$\cmark$ & \cellcolor{verylightblue}$\cmark$ & \cellcolor{verylightblue}$\cmark$ & \cellcolor{verylightblue}$\cmark$ \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Comparisons of typical methods for calibration.}
%     \label{tab:calibration_comparison}
%     \vspace{-5pt}
% \end{table}



% \begin{table}[h]
%     \centering
%     \renewcommand{\arraystretch}{1.2}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{llcccc}
%         \toprule
%         \multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Calibration Method}} & \multirow{2}{*}{\textbf{No Source \\ Data}} & \multirow{2}{*}{\textbf{No Extra \\ Training}} & \multirow{2}{*}{\textbf{Instance-wise \\ Calibration}} & \multirow{2}{*}{\textbf{Quality of \\ Candidate}}
%         \midrule
%         \multirow{3}{*}{TS} & Vanilla TS  & \textcolor{red}{$\times$} & \textcolor{red}{$\times$} & \textcolor{blue}{$\checkmark$} & \textcolor{red}{$\times$} \\
%         & TransCal  & \textcolor{red}{$\times$} & \textcolor{red}{$\times$} & \textcolor{blue}{$\checkmark$} & \textcolor{red}{$\times$} \\
%         & PseudoCal  & \textcolor{blue}{$\checkmark$} & \textcolor{red}{$\times$} & \textcolor{blue}{$\checkmark$} & \textcolor{red}{$\times$} \\
%         \midrule
%         \multirow{2}{*}{Ensemble} & MC Dropout  & \textcolor{blue}{$\checkmark$} & \textcolor{blue}{$\checkmark$} & \textcolor{red}{$\times$} & \textcolor{blue}{$\checkmark$} \\
%         & SICL (Ours)  & \textcolor{blue}{$\checkmark$} & \textcolor{blue}{$\checkmark$} & \textcolor{blue}{$\checkmark$} & \textcolor{blue}{$\checkmark$} \\
%         \bottomrule
%     \end{tabular}}
%     \caption{Comparison of calibration methods based on various criteria.}
%     \label{tab:calibration_comparison}
% \end{table}



%\noindent\textbf{Model Calibration.} 

\begin{table}[t!]
    \centering
    \tiny % Reduce font size
    \renewcommand{\arraystretch}{1} % Adjust row height for readability
    \setlength{\tabcolsep}{1pt} % Adjust column spacing
    \resizebox{\columnwidth}{!}{  
    \begin{tabular}{>{\centering\arraybackslash}p{1cm} |>{\centering\arraybackslash}p{1.2cm} >{\centering\arraybackslash}p{1cm} >{\centering\arraybackslash}p{1.2cm} >{\centering\arraybackslash}p{1.2cm} >{\centering\arraybackslash}p{1.2cm}}
        \toprule
        \textbf{Category} & \textbf{Calibration Method} & \textbf{No Source Data} & \textbf{No Extra Training} & \textbf{Instance-wise Calibration} & \textbf{Quality of Ensemble Candidate} \\
        \midrule
        \multirow{3}{*}{\makecell{Temperature \\Scaling}} & Vanilla TS  & \cellcolor{verylightred}$\xmark$ & \cellcolor{verylightred}$\xmark$& \cellcolor{verylightred}$\xmark$ & - \\
        % & Entropy TS  & \cellcolor{verylightblue}$\cmark$ & \cellcolor{verylightred}$\xmark$& \cellcolor{verylightred}$\xmark$ & - \\
        & TransCal  & \cellcolor{verylightred}$\xmark$ & \cellcolor{verylightred}$\xmark$ & \cellcolor{verylightred}$\xmark$ & - \\
        & PseudoCal  & \cellcolor{verylightblue}$\cmark$& \cellcolor{verylightred}$\xmark$ & \cellcolor{verylightred}$\xmark$ & - \\
        \midrule
        \multirow{2}{*}{Ensembling} & MC Dropout  & \cellcolor{verylightblue}$\cmark$ & \cellcolor{verylightblue}$\cmark$ & \cellcolor{verylightblue}$\cmark$ & Low \\
        & \textbf{SICL (Ours)}  & \cellcolor{verylightblue}$\cmark$ & \cellcolor{verylightblue}$\cmark$ & \cellcolor{verylightblue}$\cmark$ & High \\
        \bottomrule
    \end{tabular}}
    \caption{Comparison of calibration methods.}
    \label{tab:calibration_comparison}
    \vspace{-10pt}
\end{table}

\paragraph{Test-Time Adaptation.} 
The goal of Test-Time Adaptation (TTA) is to adapt deployed models to distributional shifts encountered during inference without access to labeled target data. Typical TTA methods~\cite{tent,chen2022contrastive,liang2020we, memo} use techniques like entropy minimization, pseudo-labeling, and target-specific feature refinement to respond to these shifts. Recently, interest has surged in more practical TTA methods~\cite{sotta,rotta,cotta,note,sar,niu2023towards} designed for real-world test streams (e.g., continual shifts, noisy streams). However, a key limitation of existing TTA methods is their tendency toward overconfidence, leading to unreliable confidence estimates—a problem that becomes even more severe in dynamic test streams (Section \ref{sec:observation}). This unreliability poses significant risks in high-stakes decision making scenarios. These challenges highlight the need for robust uncertainty estimation in TTA to ensure reliability. To address these similar concerns, AETTA~\cite{Lee_2024_CVPR} introduced dropout to estimate accuracy. However, dropout generates low-quality ensemble candidates with distorted content, resulting in ineffective uncertainty estimation (Section \ref{sec:content_analysis}).




%\input{ICCV2025-Author-Kit-Feb/figs/backgrounds}

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/3_preliminaries.tex <==
\input{wacv-2026-author-kit-template/figs/observation}
\section{Preliminaries}\label{sec:background} 


% \paragraph{Test-Time Adaptation (TTA)} 
% Test-Time Adaptation (TTA) \cite{tent, eata, sar,rotta, sotta} aims to improve model performance on test data from a distribution different from the training data by updating model parameters at inference time. 
% Given an online model \( f_{\theta_t} \), where \( \theta_t \) represents the model parameters at time step \( t \), and a test data stream \( \{ \mathbf{x}_t \}_{t=1}^T \), the model receives an online test batch \( \mathbf{x}_t \) at each time step \( t \). It first updates the parameters \( \theta_t \) based on \( \mathbf{x}_t \) and then makes a prediction \( \hat{y}_t = f_{\theta_t}(\mathbf{x}_t) \) in an online manner. 
% The goal of TTA is to ensure that the deployed model \( f_{\theta_t} \) remains accurate and adaptable, even as it encounters unlabeled test data from an unknown distribution that may shift over time.

\paragraph{Style-Content Differentiation in Representation Learning}
We revisit the style-content assumptions of representation learning~\cite{mitrovic2020representation, von2021self} and ideal properties in an adapted model. The assumptions underpinning our research motivation (Section ~\ref{sec:motivation}) are as follows.
\begin{itemize}
    \item \textbf{Data Generation from Style and Content}: Data is generated from two distinct variables—content and style—where only content is pertinent to downstream tasks, while style introduces irrelevant variations.
    \item \textbf{Independence of Content and Style}: Content and style are independent variables, and style transformations do not alter the underlying content of the data.
    % \item \textbf{Content-driven Prediction}: If the adapted model has learned appropriate representations, it makes predictions based on content rather than style.
    \item \textbf{Content-driven Prediction}: An ideal machine learning model makes its predictions based on content rather than style.
     % \item \textbf{Content-driven Prediction}: As shown in Figure \ref{Fig:backgrounds}, if the adapted model has learned appropriate representations, it makes predictions based on content rather than style.
    % \item \textbf{Style and Content Statistics}: In both CNNs and Vision Transformers, deeper layers tend to encode more content-oriented information rather than style.
\end{itemize}
We believe this assumption is valid in most practical scenarios, as empirically evidenced in Section~\ref{sec:ablation}. Furthermore, in situations where the model cannot distinguish a sample’s content from its style completely (\textit{i.e.}, model collapse), addressing this issue requires adaptation rather than calibration, as calibration alone cannot correct the fundamental inaccuracies within the model.

% For a situation where the assumption does not hold (\textit{i.e.,} model collapse), it becomes an issue that should be addressed through adaptation methods rather than calibration since calibration cannot handle fundamental inaccuracies in the underlying model.

% \paragraph{Calibration in TTA}
% To carry out predictive uncertainty calibration in TTA, the model’s predictions are calibrated for each online batch after model updates, ensuring that predictions remain reliable as the model adapts to new distributions. For each test batch at time step \( t \), the predicted confidence \( \text{conf}^{(t)} \) and accuracy \( \text{acc}^{(t)} \) are recorded and accumulated from the beginning to the current time, providing a basis for cumulative calibration error. 
% Here, we define Cumulative Expected Calibration Error (ECE) specifically for TTA scenarios, extending the standard ECE definition~\cite{naeini2015obtaining} to quantify the discrepancy between confidence and accuracy over time by aggregating online model's predictions at each time step.
% The Cumulative ECE can be expressed as:

% \begin{equation}
% \begin{aligned}
%      \frac{1}{n_T} \! \sum_{t=1}^{n_T} \sum_{k=1}^{K} \frac{|B_k^{(t)}|}{N^{(t)}} \left| \text{acc}_k^{(t)} - \text{conf}_k^{(t)} \right|,
% \end{aligned}
% \end{equation}
% % \begin{equation}
% % \begin{aligned}
% %      \frac{1}{T} \! \sum_{i=1}^N  \! h({X} ; \Theta) \neq {h}({X} ; \Theta^{{\tt dropout}_i}),
% % \end{aligned}
% % \end{equation}
% where \( n_T \) represents the total number of test batches,  \( K \) is the number of confidence bins, \( B_k^{(t)} \) is the set of samples in bin \( k \) during the \( t \)-th batch, \(  \text{acc}_k^{(t)}\) and \( \text{conf}_k^{(t)} \) are the accuracy and average confidence of  \( B_k^{(t)} \) and \( N^{(t)} \) is the total number of samples in the \( t \)-th batch. This formulation allows continuous monitoring of calibration quality over time, supporting TTA scenarios where high confidence alignment with accuracy is critical.
% Note that all the calibration errors reported in this paper are cumulative ECE.

% Cumulative Expected Calibration Error (ECE) then quantifies the discrepancy between confidence and accuracy over time by aggregating predictions in each confidence bin. 




==> sec/4.5_motivation.tex <==
\section{Motivation}\label{sec:motivation}
\input{figs/motivation}

In the TTA scenario, the aforementioned challenges fundamentally arise because the distribution of the test stream can change very dynamically. In this respect, instance-wise calibration through \textit{ensembling} is more appropriate than \textit{temperature-scaling} approaches~\cite{guo2017calibration, wang2020transferable, park2020calibrated, hupseudo} that scale with a single temperature for a fixed distribution. Moreover, \textit{temperature-scaling} methods require additional data and training for obtaining the temperature parameter, which is undesirable in TTA. For \textit{ensemble-based} calibration, the quality of ensemble candidates is crucial for the uncertainty estimation. However, the quality of ensemble candidate representations remains suboptimal in state-of-the-art \textit{ensembling} approach, MC Dropout~\cite{dropout}.
% However, the representative ensemble-based methods, MC Dropout~\cite{dropout}, the quality of ensemble candidate representations is suboptimal.
To realize proper instance-wise calibration with ensembling, confidence should be estimated through consistency with ensemble candidates where only the style is changed while preserving the content defining the instance itself. However, dropout could generate poor candidate representations since the process of randomly disabling neurons, which often includes informative nodes, results in representations that lose critical content information.


Here, we provide a motivative analysis of the candidate embeddings $\mathbf{z}_i$ of the target image instance $\mathbf{x}_i$ from CIFAR10-C. First, we provide insights on the necessity of preserving the content for candidate representation. Upon this, we offer comparison for candidate representation  produced by MC Dropout~\cite{dropout} and style-shifted representation from MixStyle~\cite{zhou2021domain}, a representative style-variation method.

\input{figs/main_figure}
% Here, we provide a detailed analysis of the candidate embeddings $\mathbf{z}_i$ of the target image instance $\mathbf{x}_i$ from CIFAR10-C. First, we provide insights on the necessity of preserving the content for candidate representation. Upon this, we offer comparative analysis for candidate representation with embeddings produced by MC Dropout~\cite{dropout} and style-shifted representation from MixStyle~\cite{zhou2021domain}, a representative method for generating style-variants at the feature level.

% Here, we provide a detailed analysis of the candidate embeddings $\mathbf{z}_i$ produced by MixStyle~\cite{zhou2021domain}. First, we provide insights on the necessity of preserving the content during the ensembling of predictions. Upon this, we provide comparative results with MC Dropout~\cite{gal2016dropout}, demonstrating that SICL effectively preserves the content while only altering the style.

\subsection{Ideal Characteristics of Ensemble Candidates}\label{sec:ideal_ensemble}

Here, we empirically validate our assumption that optimal ensemble candidates should be (1) style-variant and (2) content-preserving. Figure~\ref{Fig:motivation} (a) presents our results.
We visualize the effect of ensembling 20 different candidates generated via (1) \textit{Style Perturbation}, adding gaussian noise into style statistics (channel-wise mean $\mu_i$ and standard deviation $\sigma_i$ of earlier layer feature $\mathbf{z}_i$ of ResNet, following the seminal style-transfer works~\cite{huang2017arbitrary, dumoulin2017learned, Gatys_2016_CVPR, ulyanov2016instance}) and (2) \textit{Content Perturbation}, appling perturbations to the embeddings' content rather than style. Specifically, we add Gaussian noise to whitened features $\frac{\mathbf{f}_i - \mu_i}{\sigma_i}$ and then restoring them to $\mu_i$ and $\sigma_i$. Building on prior studies~\cite{huang2017arbitrary, pan2018two} that identify whitened features as a content representation, our results show that content corruption leads to severe calibration errors, over 4 times higher than with style perturbations, highlighting the importance of separating style to preserve the content during the ensemble candidate generation process.



\subsection{Embedding-level Comparative Analysis}\label{sec:content_analysis}
%\paragraph{Embedding-level Analysis between MC Dropout and MixStyle.}
% In Figure~\ref{Fig:qualitative_analysis} (b), we can observe that the style-shifted ensemble candidates generated through MixStyle preserve content information significantly better than candidates generated via MC Dropout, regardless of various corruptions.
% To determine whether ensemble candidates generated by dropout effectively preserve the content information of an instance, we introduced MixStyle, a representative method for generating style-variants at the feature level, and conducted a comparative analysis.

% To quantify content preservation, we measure how well the candidate embeddings maintain their geometric relationship with class centroids, comparing style-shifted embeddings against with MC Dropout generated embeddings. Specifically, for each instance $i$, we compute the Mahalanobis distance~\cite{mahalanobis2018generalized} between its embedding and the corresponding class centroid $\boldsymbol{\mu}_c$, denoted as $\mathbf{D}_c(\mathbf{z}_i) = \sqrt{(\mathbf{z}_i - \boldsymbol{\mu}_c)^T \mathbf{\Sigma}_c^{-1} (\mathbf{z}_i - \boldsymbol{\mu}_c)}$. We then calculate the same distance for its candidate embedding ($z_i^\text{cand}$). The content preservation metric, $\Delta \mathbf{D}_{c}^{\text{cand}}$, is defined as the average absolute difference between these distances across $N$ samples: $\frac{1}{N} \sum_{i=1}^{N} \left| \mathbf{D}_c\left(\mathbf{z}_i\right) - \overline{\mathbf{D}}_c\left(\mathbf{z}_i^{\text{cand}}\right) \right|$. By leveraging the Mahalanobis distance, $\mathbf{D}_{c}^{\text{cand}}$ accounts for the covariance structure of the embedding space, enabling a more faithful measurement of distances compared to standard Euclidean metrics. The evaluation of $\Delta \mathbf{D}_{c}^{\text{cand}}$ across 15 corruption types in CIFAR10-C is presented in Figure~\ref{Fig:motivation}(b). The results demonstrate that style-shifted embeddings consistently achieves significantly lower $\Delta \mathbf{D}_{c}^{\text{cand}}$ values compared to MC Dropout, indicating its superior capability in preserving content-related features. 

% Based on the intuition that a candidate embedding that well-preserves its content shall retain their geometric relationship to the embedding of its class centroid, we compare style-shifted embeddings with those generated by MC Dropout via Mahalanobis distance. Specifically, for each sample $i$, we compute the Mahalanobis distance $\mathbf{D}_c(\mathbf{z}_i) = \sqrt{(\mathbf{z}_i - \boldsymbol{\mu}_c)^T \mathbf{\Sigma}_c^{-1} (\mathbf{z}_i - \boldsymbol{\mu}_c)}$ between its original embedding $\mathbf{z}_i$ and the corresponding class centroid $\boldsymbol{\mu}c$. We then measure the same distance for its candidate embedding $\mathbf{z}i^{\text{cand}}$. By taking the average absolute difference between the two distances across N samples, we quantify the content preservation of the candidate embeddings, concretely as follows:
% \[
% \Delta \mathbf{D}{c}^{\text{cand}}=\frac{1}{N} \sum_{i=1}^{N} \left| \mathbf{D}_c\left(\mathbf{z}_i\right) - \overline{\mathbf{D}}_c\left(\mathbf{z}_i^{\text{cand}}\right) \right|
% \]
% Note that, through Mahalanobis distance, we account for the covariance structure in the embedding space—leading to a more reliable measure of how well the candidate embeddings preserve content-related features. Figure~\ref{Fig:motivation}(b) shows the results of $\Delta \mathbf{D}{c}^{\text{cand}}$ evaluated over 15 corruption types in CIFAR10-C. Across all corruptions, style-shifted embeddings achieve substantially lower $\Delta \mathbf{D}{c}^{\text{cand}}$ values than MC Dropout embeddings, highlighting their superior ability to maintain the original content structure.



Based on the intuition that a candidate embedding that well-preserves its content shall retain their geometric relationship to the embedding of its class centroid, we compare style-shifted embeddings with those generated by MC Dropout via Mahalanobis distance. Specifically, for each sample $\mathbf{x}_i$ and its $N$ ensemble candidates $\mathbf{z'}_{i,j}$, we compute the Mahalanobis distance $\mathcal{D}_M(\mathbf{z}_i) = \sqrt{(\mathbf{z}_i - \boldsymbol{\mu}_c)^T \mathbf{\Sigma}_c^{-1} (\mathbf{z}_i - \boldsymbol{\mu}_c)}$ between its original embedding $\mathbf{z}_i$ and the corresponding class centroid $\boldsymbol{\mu}_c$. Here, we define \textit{ContentVariance} of candidate embedding $\mathbf{z'}_{i}$ as follows:

\[
\textit{ContentVariance}(\mathbf{z'}_i)= \left| \mathcal{D}_M\left(\mathbf{z}_i\right) - \frac{1}{N} \sum_{j=1}^{N}{\mathcal{D}}_M\left(\mathbf{z'}_{i,j}\right) \right|
\]
Note that, through Mahalanobis distance, we account for the covariance structure in the embedding space—leading to a more reliable measure of how well the candidate embeddings preserve content-related features. Figure~\ref{Fig:motivation}(b) shows the results of average \textit{ContentVariance} for all samples in CIFAR10-C. Across all corruptions, style-shifted embeddings achieve substantially lower \textit{ContentVariance} than MC Dropout embeddings, highlighting their superior ability to maintain the original content information.



% Based on the intuition that a candidate embedding that well-preserves its content shall retain their geometric relationship to the embedding of its class centroid, we compare style-shifted embeddings with those generated by MC Dropout via Mahalanobis distance. Specifically, for each sample $\mathbf{x}_i$ and its $N$ ensemble candidates $\mathbf{x'}_{i,j}$, we compute the Mahalanobis distance $\mathbf{D}_c(\mathbf{z}_i) = \sqrt{(\mathbf{z}_i - \boldsymbol{\mu}_c)^T \mathbf{\Sigma}_c^{-1} (\mathbf{z}_i - \boldsymbol{\mu}_c)}$ between its original embedding $\mathbf{z}_i$ and the corresponding class centroid $\boldsymbol{\mu}_c$. We then measure the same distance for its candidate embedding $\mathbf{z'}_{i,j}$. 

% %By taking the average absolute difference between the two distances across N samples

% we quantify the content preservation of the candidate embeddings, concretely as follows:
% \[
% \Delta \mathbf{D}_{c}(\mathbf{z}_i)= \left| \mathbf{D}_c\left(\mathbf{z}_i\right) - \frac{1}{N} \sum_{j=1}^{N}{\mathbf{D}}_c\left(\mathbf{z'}_{i,j}\right) \right|
% \]
% Note that, through Mahalanobis distance, we account for the covariance structure in the embedding space—leading to a more reliable measure of how well the candidate embeddings preserve content-related features. Figure~\ref{Fig:motivation}(b) shows the results of average $\Delta \mathbf{D}_{c}(\mathbf{z}_i)$ evaluated over 15 corruption types in CIFAR10-C. Across all corruptions, style-shifted embeddings achieve substantially lower $\Delta \mathbf{D}_{c}(\mathbf{z}_i)$ values than MC Dropout embeddings, highlighting their superior ability to maintain the original content structure.


 %while effectively altering style attributes.

% Furthermore, we visualize the variability of the generated embeddings $z_i$ on Figure~\ref{Fig:qualitative_analysis} (c). Here, we plot the mean variance of candidate embeddings of each sample in the CIFAR-10C dataset. It can be seen that the style-perturbed embeddings from SICL exhibit a higher variability across most (14/15) corruption types. Thus, we find SICL to generate proper candidate embeddings that 1) maintain content integrity while 2) exhibiting higher diversity, enabling reliable and accurate prediction of model's confidence.


==> sec/4_observation.tex <==



\section{Challenges in Calibration under TTA} 

\label{sec:observation}
In this section, we examine the unique characteristics of calibration within the TTA framework. Unlike the typical environment addressed by conventional calibration approaches, TTA operates in a dynamic setting where the model continuously adapts to unseen distribution shifts without assuming a fixed test distribution, nor a fixed model state during calibration. Specifically, we find that in such dynamic settings, (1) we cannot expect consistent and reliable calibration performance in such dynamic distributions (Section~\ref{sec:difficulty-calibration}), and (2) most TTA methods~\cite{tent, sotta, sar, rotta} inadvertently push the model toward overconfidence as it adapts. (Section~\ref{sec:importance-realistic}).

% In practical test-time adaptation scenarios, achieving reliable uncertainty estimation is particularly challenging. This section outlines key observations demonstrating why maintaining robust calibration is difficult in TTA environments, where dynamic and continuous shifts necessitate an adaptive accurate confidence estimation framework. 

%These challenges underscore the importance of developing methods that can provide stable and reliable calibration in diverse and evolving test conditions.

\subsection{Calibration Instability in Test-Time Adaptation}\label{sec:difficulty-calibration}
Figure~\ref{Fig:observation} (a,b) demonstrates how distribution shifts affect calibration performance. We analyze calibration metrics while transitioning between 15 corruption types (\textit{i.e.}, Gaussian noise $\rightarrow$ Shot noise $\rightarrow$ Impulse noise ..) with a fixed model. The reliability diagrams for the initial and final 1,000 samples (Figure~\ref{Fig:observation} a) reveal markedly different patterns, despite similar Expected Calibration Error (ECE) values of approximately 20\%. Figure~\ref{Fig:observation} (b) tracks the expected calibration error using a sliding window analysis during corruption type transitions, where we find substantial fluctuations. These observations suggest that traditional calibration methods, which assume a static test distribution, will inadvertently yield unreliable performance when faced with dynamic distribution shifts, as their effectiveness becomes heavily dependent on the characteristics of the current input batch.  


% We illustrate the impact of distribution shift on calibration performance by plotting the calibration error across varying shift severities in the CIFAR10-C dataset in the Figure~\ref{fig:calibration_overview}. 
% Regardless of prediction correctness, calibration error rises consistently with increasing shift severity, as models tend to misinterpret novel samples as previously learned representations when shifts deviate further from the training distribution.
% This observation highlights the limitations of fixed `one-size-fits-all' calibration methods for handling distributional changes encountered during test-time adaptation.


% the calibration error consistently rises as the style shift degree increases, regardless of prediction correctness since models increasingly confuse novel samples with previously learned representations as these shifts diverge further from seen shifts
% highlighting that a fixed “one-size-fits-all” calibration method is inadequate for handling distributional changes encountered during test-time adaptation.

%Calibration errors are displayed separately for correct and incorrect samples. 

% As the figure reveals, calibration performance consistently worsens for both cases, highlighting that a fixed “one-size-fits-all” calibration method is inadequate for handling distributional changes encountered during test-time adaptation.

% To find the relationship between the severity of distribution shift with calibration error, we visualize the calibration error (ECE error) for correct and incorrect samples, while varying the severity   


% Deployed models frequently encounter various unseen shifts in real-world environments. As these shifts diverge further from seen shifts, models increasingly confuse novel samples with previously learned representations, leading to overconfident predictions on out-of-distribution data.

% As shown in Figure \ref{fig:correct_samples} and \ref{fig:incorrect_samples}, in a dynamic stream of CIFAR-10C, the calibration error consistently rises as the style shift degree increases, regardless of prediction correctness. This trend highlights the difficulty of achieving reliable confidence estimates during test-time adaptation as models face more severe unseen shifts.

\subsection{Continuous Adaptation Causes Overconfidence}\label{sec:importance-realistic}

The impact of model adaptation on calibration performance is illustrated in Figure~\ref{Fig:observation} (c,d). During Test-Time Adaptation (TTA), models continuously adapt to novel distributions through online learning, primarily utilizing Entropy Minimization (EM) objectives~\cite{tent, sar, sotta, rotta}. However, EM-based adaptation can lead to excessive reliance on the model's internal predictions, resulting in overconfidence. Figure~\ref{Fig:observation} (c) compares reliability diagrams between the initial and final models after TENT~\cite{tent} adaptation on CIFAR-10C Gaussian noise, revealing a threefold increase in calibration errors due to heightened overconfidence. Figure~\ref{Fig:observation} (d) tracks this degradation through sliding window analysis, showing monotonic increases in calibration loss during EM-based updates. These findings demonstrate that entropy minimization, despite its prevalence in TTA methods, systematically drives models toward overconfidence, even under static test distributions. This is consistent with the finding of the Entropy Enigma~\cite{press2024entropy} that updates through EM ultimately fail.


% We illustrate the shift in calibration performance during TTA (using TENT~\cite{tent}) on CIFAR10-C with Gaussian noise in Figure~\ref{fig:calibration_overview}. As shown in Figure~\ref{fig:avg_confidence}, the average confidence progressively increases throughout the adaptation process. Visualizing the reliability diagram after adaptation reveals a significant overconfidence bias in the model, despite improved accuracy. This trend is consistent across TTA methods due to their inherent reliance on entropy minimization~\citep{tent, sotta, rotta, sar}, which pushes the model to make increasingly confident predictions. This underscores the challenge of maintaining reliable uncertainty estimates in TTA, where models reinforce their own predictions without external supervision.


% In Test-Time Adaptation (TTA), since target data labels are inaccessible, methods like entropy minimization are used, and the model is continuously updated to address distribution shifts. However, this continual adaptation without external supervision leads the model to make increasingly overconfident predictions without adequately capturing uncertainty. 
% Figure \ref{fig:reliability_diagram} shows the reliability diagram for CIFAR-10C test samples of gaussian noise after test-time adaptation when TENT~\cite{tent} is completed, revealing an overconfident tendency across all confidence bins. Under the same setup, Figure \ref{fig:avg_confidence} shows that predictions become overconfident as adaptation goes on. This finding shows the challenge of maintaining reliable uncertainty estimates in test-time adaptation, where models continuously reinforce self-supervision in the absence of external guidance.

% These observations highlights the challenge of accurately reflecting uncertainty in test-time adaptation, where models continuously reinforce self-supervision in the absence of external guidance while facing various unseen distribution shifts.

These observations underscore the inherent challenges in achieving robust calibration in TTA, highlighting the need for tailored calibration approaches that can address evolving, unpredictable conditions without external supervision.


% These observations highlight the inherent challenges in achieving robust calibration for TTA, emphasizing the importance of tailored approaches that can address evolving, unpredictable conditions without external supervision.


%collectively
% As shown in figure \ref{fig:avg_confidence}, average prediction confidence consistently rises as the adaptation goes on, highlighting the challenge of producing confidence estimates that properly reflect uncertainty during test-time adaptation.



==> sec/5_method.tex <==
\section{Methodology}\label{sec:method}


Through the analysis in Section \ref{sec:motivation}, we recognize that the current \textit{ensemble-based} calibration methods represented by MC Dropout are insufficient to solve the challenges presented in Section \ref{sec:observation}. Therefore, we propose a methodology that generates better ensemble candidate representations based on the style-content assumptions in Section \ref{sec:background}. Building on these assumptions, we present that style invariance can serve as a robust estimator of correctness likelihood by proposing SICL in scenarios lacking label information from target domains. The overall framework of SICL is visualized in Figure \ref{Fig:main_figure}. In the following subsection, we describe the SICL by outlining the overall procedure (Section \ref{sec:method-sicl}), the generation of style variants through feature perturbation (Section \ref{sec:method-style variation}), and a relaxation mechanism to address overconfidence during model collapse (Section \ref{sec:method-relaxation}). 

% Through the analysis in Section \ref{sec:motivation}, we recognize that the current \textit{ensemble-based} calibration methods represented by MC Dropout are insufficient to solve the challenges presented in Section \ref{sec:observation}. Therefore, we propose a methodology that generates better ensemble candidate representations based on the style-content assumptions in Section \ref{sec:background}. Building on these assumptions, we present that style invariance can serve as a robust estimator of correctness likelihood by proposing SICL in scenarios lacking label information from target domains. The overall framework of SICL is visualized in Figure \ref{Fig:main_figure}. In the following subsection, we describe the SICL by detailing the measurement of style invariance (Section \ref{sec:method-sicl}), the generation of style variants through feature perturbation (Section \ref{sec:method-style variation}), and a relaxation mechanism to address overconfidence during model collapse (Section \ref{sec:method-relaxation}). 

%The SICL framework is summarized in Figure~\ref{Fig:main_figure}.

% As highlighted in Section~\ref{sec:motivation}, embeddings generated via MC-Dropout often blindly corrupt the content of input samples. To overcome this, we propose SICL, a novel calibration method for TTA grounded in style-content assumptions (Section~\ref{}). SICL assigns sample-level confidence by multiplying two complementary metrics: (1) the style invariance ratio $\gamma^{\text{style}}_i$, favoring predictions robust to \textit{style perturbations}, and (2) the content invariance ratio $1 - \gamma^{\text{content}}_i$, penalizing predictions sensitive to \textit{content perturbations}. We detail the computation of overall sample confidence (Section~\ref{sec:method-sicl}), style invariance (Section~\ref{sec:method-style variation}), and content invariance ratios (Section~\ref{sec:method-relaxation}). The SICL framework is summarized in Figure~\ref{Fig:main_figure}.



% To this end, we propose SICL, a novel method to calibrate models under Test-time Adapation through the lens of  style invariance.

% Motivated by Section~\ref{sec:motivation}, we propose SICL, a novel method to calibrate models under Test-time Adaptation. Grounded on the style-content assumptions (Section~\ref{sec:background})




%To address the challenges outlined in Section \ref{sec:observation}, 
% Through the analysis in Section \ref{sec:motivation}, we recognize that the current \textit{ensemble-based} calibration methods represented by MC Dropout are insufficient to solve the challenges presented in Section \ref{sec:observation}. Therefore, we propose a methodology that generates better ensemble candidate representations based on the style-content assumptions in Section \ref{sec:background}. Building on these assumptions, we present that style invariance can serve as a robust estimator of correctness likelihood by proposing SICL in scenarios lacking label information from target domains. The overall framework of SICL is visualized in Figure \ref{Fig:main_figure}.


% In the following subsection, we outline the SICL by detailing the measurement of style invariance (Section \ref{sec:method-sicl}), the generation of style variants through feature perturbation (Section \ref{sec:method-style variation}), and a relaxation mechanism to address overconfidence during model collapse (Section \ref{sec:method-relaxation}).



% To address the challenges outlined in Section \ref{sec:observation}, we revisit the assumptions of representation learning~\cite{mitrovic2020representation, von2021self} and style-content statistics of vision models.

% The assumptions underpinning our method are as follows.
% \begin{itemize}
%     \item \textbf{Data Generation from Style and Content}: Data is generated from two distinct variables—content and style—where only content is pertinent to downstream tasks, while style introduces irrelevant variations.
%     \item \textbf{Independence of Content and Style}: Content and style are independent variables, and style transformations do not alter the underlying content of the data.
%     \item \textbf{Content-driven Prediction}: If the adapted model has learned appropriate representations, it makes predictions based on content rather than style.
%     % \item \textbf{Style and Content Statistics}: In both CNNs and Vision Transformers, deeper layers tend to encode more content-oriented information rather than style.
% \end{itemize}

% We believe this assumption is valid in practical scenarios. For a situation where the assumption does not hold (\textit{i.e.,} model collapse), it becomes an issue that should be addressed through adaptation methods rather than calibration since calibration cannot handle fundamental inaccuracies in the underlying model. Building on these assumptions, we present that style invariance can serve as a robust estimator of correctness likelihood by proposing SICL in scenarios lacking label information from the source or target domains. The overall framework of SICL is visualized in Figure \ref{Fig:main_figure}.


% In the following subsection, we outline the SICL by detailing the measurement of style invariance (Section \ref{sec:method-sicl}), the generation of style variants through feature perturbation (Section \ref{sec:method-style variation}), and a relaxation mechanism to address overconfidence during model collapse (Section \ref{sec:method-relaxation}).


\subsection{Style Invariance as a Correctness Likelihood}\label{sec:method-sicl}
% Under the given assumptions stated in the Section \ref{sec:background}, a prediction that is insensitive to perturbations in style indicate that the model is making predictions based more on the content, and is thus likely to be confident. Conversely, a prediction that 



%\subsection{Style Invariance as a Correctness Likelihood}\label{sec:method-sicl}

Given an original sample \( \mathbf{x}_i \), its feature  \( \mathbf{z}_i \) and a trained model \( f \), we calculate the final prediction confidence by measuring instance-wise style invariance, with an additional relaxation term to handle non-ideal cases. To do this, we perform the following steps:

% Given an original sample \( \mathbf{x}_i \) and a trained model \( f \) capable of capturing semantic contents, we aim to estimate the correctness likelihood of the model's prediction with an instance-wise style invariance and use it as a final prediction confidence. To do this, we perform the following steps:

% Given an original sample \( \mathbf{x}_i \) and a trained model \( f \) capable of capturing semantic contents, we aim to estimate the correctness likelihood of the model's prediction with an instance-wise style invariance and use it as a final prediction confidence for robust calibration. To do this, we perform the following steps:


\begin{enumerate}
    \item \textbf{Generating Style Variants}: Create a set of \( N \) style-transformed samples \( \{ \mathbf{z}_{i,j}^{s\prime} \}_{j=1}^{N} \) as ensemble candidates
    by applying different style transformation \( T \) with style \( s_j \) to the \( \mathbf{z}_i \), resulting in 
   \( \mathbf{z}^{s\prime}_{i,j} = T(\mathbf{z}_i, s_j), \quad \forall j \in \{1, \dots, N\}. \)
    The style transformation \( T \) alters the style while preserving the content.

    \item \textbf{Measuring Style Invariance as a Initial Confidence}: Calculate the style invariance ratio \( \gamma^{style}_i \) as initial prediction confidence $p_{\text{init.}}(y_i)$ with the prediction consistency between the original prediction \( \hat{y_i} = f(\mathbf{x}_i) \) and the predictions on the style variants \( \{ y_{i,j}^{s\prime} \}_{j=1}^{N} \). Concretely,
    \[
    p_{\text{init.}}(y_i) = \gamma^{style}_i = \frac{1}{N} \sum_{j=1}^{N} \mathbb{I}\left( \hat{y}_i = \hat{y}^{s\prime}_{i,j} \right)
    \]
    where \( \mathbb{I} \) is the indicator function.

    \item \textbf{Handling Potential Collapse with Relaxation}: We derive $p_{\text{init.}}(y_i)$ based on the assumption that models perform content-driven prediction. However, this may not always hold in practical scenarios. To address this, we compute the final calibrated confidence by applying relaxation $\omega_\text{relaxation}$, which mitigates the overconfidence arising from the model collapses. This can be formulated as follows:
    \[
    p_{\text{calibrated}}(y_i) = \omega_\text{relaxation}\cdot p_{\text{init.}}(y_i)
    \]

    % \item \textbf{Measuring Prediction Consistency}: Calculate the prediction consistency ratio \( \gamma_i \) between the original prediction \( \hat{y_i} = f(\mathbf{x}_i) \) and the predictions on the style variants \( \{ y_{i,j}^{\prime} \}_{j=1}^{N} \). This can be quantified using a proportion of matching predictions:
    % \[
    % \gamma_i = \frac{1}{N} \sum_{j=1}^{N} \mathbb{I}\left( \hat{y}_i = \hat{y}_{i,j}' \right)
    % \]
    % where \( \mathbb{I} \) is the indicator function.
\end{enumerate}
% Under the given assumptions stated in the Section \ref{sec:background}, a high style invariance ratio \( \gamma^{style}_i \) suggests that the model's prediction of sample \( \mathbf{x}_i \) is likely to be confident, as it relies on the invariant content \( c \). Conversely, a low \( \gamma^{style}_i \) indicates sensitivity to style changes, implying lower confidence in the prediction $\hat{y}_i$. 

% \begin{enumerate}
%     \item \textbf{Generating Style Variants}: Create a set of \( N \) style-transformed samples \( \{ \mathbf{x}_{i,j}^{\prime} \}_{j=1}^{N} \) as ensemble candidates
%     by applying different style transformation \( T \) with style \( s_j \) to the \( \mathbf{x}_i \), resulting in 
%    \( \mathbf{x}_{i,j}' = T(\mathbf{x}_i, s_j), \quad \forall j \in \{1, \dots, N\}. \)
%     The style transformation \( T \) alter the style while preserving the content.

%     \item \textbf{Predicting on Style Variants}: Obtain predictions for each style-transformed sample: \( \hat{y}_{i,j}' = f(\mathbf{x}_{i,j}') \).

%     \item \textbf{Measuring Prediction Consistency}: Calculate the style invariance ratio \( \gamma^{style}_i \) with the the prediction consistency between the original prediction \( \hat{y_i} = f(\mathbf{x}_i) \) and the predictions on the style variants \( \{ y_{i,j}^{\prime} \}_{j=1}^{N} \). This can be quantified using a proportion of matching predictions:
%     \[
%     \gamma^{style}_i = \frac{1}{N} \sum_{j=1}^{N} \mathbb{I}\left( \hat{y}_i = \hat{y}_{i,j}' \right)
%     \]
%     where \( \mathbb{I} \) is the indicator function.
%     % \item \textbf{Measuring Prediction Consistency}: Calculate the prediction consistency ratio \( \gamma_i \) between the original prediction \( \hat{y_i} = f(\mathbf{x}_i) \) and the predictions on the style variants \( \{ y_{i,j}^{\prime} \}_{j=1}^{N} \). This can be quantified using a proportion of matching predictions:
%     % \[
%     % \gamma_i = \frac{1}{N} \sum_{j=1}^{N} \mathbb{I}\left( \hat{y}_i = \hat{y}_{i,j}' \right)
%     % \]
%     % where \( \mathbb{I} \) is the indicator function.
% \end{enumerate}
% Under the given assumptions stated in the Section \ref{sec:background}, a high style invariance ratio \( \gamma^{style}_i \) suggests that the model's prediction of sample \( \mathbf{x}_i \) is likely to be confident, as it relies on the invariant content \( c \). Conversely, a low \( \gamma^{style}_i \) indicates sensitivity to style changes, implying lower confidence in the prediction $\hat{y}_i$. 

\subsection{Style Variation through Perturbation}\label{sec:method-style variation}

Key component for measuring instance-wise style invariance is securing a style transformation \( T \) that is able to simulate realistic shift by preserving the semantic content information of instance while altering its style.  To achieve this, we extract style representation from feature statistics and generate style-variants by perturbing this representation with a Gaussian noise. We exploit the channel-wise mean $\mu$ and standard deviation $\sigma$ of a feature map as a style representation, following the seminal style-transfer works~\cite{huang2017arbitrary, dumoulin2017learned, Gatys_2016_CVPR, ulyanov2016instance}. Based on these studies demonstrating that shallow layers tend to capture significant style information, we utilize the feature representation from the first layer.
 
 For each \(\mathbf{x}_i\), we compute the channel-wise mean and standard deviation of the feature map \(\mathbf{f}_i \in \mathbb{R}^{ C \times H \times W} \) as:
\begin{equation}
\begin{aligned}
   \mu_i = \frac{1}{H \times W} \sum_{h=1}^{H} \sum_{w=1}^{W} \mathbf{f}_i^{(c, h, w)},
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
\sigma_i = \sqrt{\frac{1}{H \times W} \sum_{h=1}^{H} \sum_{w=1}^{W} \left(\mathbf{f}_i^{(c, h, w)} - \mu_i\right)^2.}
\end{aligned}
\end{equation}
To realize style perturbation, we add random noise to the original \(\mu_i\) and \(\sigma_i\) or apply modified values. The perturbed mean \(\mu_{\text{perturb}}\) and standard deviation \(\sigma_{\text{perturb}}\) are defined as:
\begin{equation}
\begin{aligned}
   \mu_{\text{perturb}} = \mu_i + \delta\epsilon_\mu, \quad \sigma_{\text{perturb}} = \sigma_i + \delta\epsilon_\sigma, 
\end{aligned}
\end{equation}
where \(\epsilon_\mu\) and \(\epsilon_\sigma  \sim \mathcal{N}(0, 1)\) are random noise which follow the standard Gaussian distribution. Here, \(\delta\) is a standard deviation of $\mu_i$ for online test batch. While a similar approach like MixStyle~\cite{zhou2021domain}, which synthesizes a new style by mixing the style statistics of two samples, it is limited by its dependency on the input batch - which is undesirable in a TTA scenario. In contrast, leveraging stochastic perturbation with Gaussian noise enables the generation of diverse style representations with varying directions and intensities, offering greater flexibility and variation (Section \ref{sec:analysis}).


Using the \(\mu_{\text{perturb}}\) and \(\sigma_{\text{perturb}}\), we generate perturbed features as style variants, denoted by  \(\mathbf{f}_{\text{perturb}}\):
\begin{equation}
\begin{aligned}
   \mathbf{f}_{\text{perturb}} = \sigma_{\text{perturb}} \cdot \frac{\mathbf{f}_i - \mu_i}{\sigma_i} + \mu_{\text{perturb}}.
\end{aligned}
\end{equation}
We use the consistency between the predictions of the 
\( N \) style variants generated from \( \mathbf{f}_{\text{perturb}} \) and the original sample's prediction as the confidence of original sample \( \mathbf{x}_i \).

% \subsection{Style Perturbation for Vision Transformers}
% For Vision Transformers, we realize our style perturbation approach on the patch embedding space. Given an input image \(\mathbf{x}_i\) processed into a sequence of patch embeddings $\textbf{p} \in \mathbb{R}^{n_{\text{patch}} \times D}$, where $n_{\text{patch}}$ is the number of patches and $D$ is the embedding dimension, we compute the patch-wise mean and standard deviation as follows:
% \begin{equation}
% \mu_i = \frac{1}{n_{\text{patch}}} \sum_{j=1}^{n_{\text{patch}}} \textbf{p}_{j,i}, \sigma_i^2 = \frac{1}{n_{\text{patch}}} \sum_{j=1}^{n_{\text{patch}}} (\textbf{p}_{j,i} - \mu_i)^2
% \end{equation}
% where $\mu_i$ represents the mean and $\sigma_i^2$ the variance across patches. As utilized in TFS-ViT~\cite{noori2024tfs}, these token-level statistics capture global style information across token positions in the embedding space. The remaining process of SICL is the same as when using CNN.

\subsection{Relaxation for Collapse}\label{sec:method-relaxation}
SICL assumes that a model effectively disentangles style and content. However, during continuous adaptation in TTA, model often falls into a collapsed state where it overly attends to the style rather than content during its predictions, hence making the style invariance term unreliable. Thus, we introduce a relaxation weight $\omega_\text{relaxation}$ that penalizes content-independent predictions that overly attend on the \textit{style}.
To identify the content-independent predictions, we calculate the content invariance ratio $\gamma^{content}_i$ which quantifies the invariance of predictions with respect to content distortion. Specifically, we calculate the content invariance ratio $\gamma^{content}_i$ as follows:
\[
\gamma^{content}_i = \frac{1}{N} \sum_{j=1}^{N} \mathbb{I}\left( \hat{y}_i = \hat{y}^{c\prime}_{i,j} \right)
\]
where $\hat{y}^{c\prime}_{i,j}$ denotes the predictions of content-distorted sample $\mathbf{z}^{c\prime}_i$. Grounded in prior works~\cite{huang2017arbitrary, pan2018two}, we obtain the whitened embeddings (content-specific embedding) to simulate content distortion  as follows: $\mathbf{f}_{\text{white}} = \frac{\mathbf{f}_i - \mu_i}{\sigma_i + \epsilon}$. Next, we add gaussian noise to perturb its content; concretely as follows:
\[
    \mathbf{f}_{\text{content-perturb}} = \sigma_i \cdot (\mathbf{f}_{\text{white}} + \mathbf{\epsilon}) + \mu_i 
\]
where, $ \mathbf{\epsilon}$ is the gaussian noise \(\epsilon_\sigma  \sim \mathcal{N}(0, \sigma^{\text{white}}_i \cdot I)\). In essence, we're applying standard gaussian noise scaled to the channel-wise standard deviations of the whitened features.
The final relaxation weight is defined as $\omega_\text{relaxation} = 1-\gamma^{content}_i$, which effectively penalizes predictions that remain unchanged despite content modifications.

% \subsection{Relaxation for Collapse}\label{sec:method-relaxation}
% SICL assumes that a model effectively disentangles style and content. However, during continuous adaptation in TTA, model often falls into a collapsed state where it overly attends to the style rather than content during its predictions, hence making the style invariance term unreliable. Thus, we introduce a relaxation weight $\omega_\text{relaxation}$ that penalizes content-independent predictions that overly attend on the \textit{style}.
% To identify the content-independent predictions, we calculate the content invariance ratio $\gamma^{content}_i$ which quantifies the invariance of predictions with respect to content distortion. Specifically, we calculate the content invariance ratio $\gamma^{content}_i$ as follows:
% \[
% \gamma^{content}_i = \frac{1}{N} \sum_{j=1}^{N} \mathbb{I}\left( \hat{y}_i = \hat{y}^{c\prime}_{i,j} \right)
% \]
% where $\hat{y}^{c\prime}_{i,j}$ denotes the predictions of content-distorted sample $\mathbf{x}^{c\prime}_i$. To simulate content distortion, we utilized the \textit{Content Perturbation} from Section \ref{sec:ideal_ensemble}. 


% The relaxation weight is defined as $\omega_\text{relaxation} = 1-\gamma^{content}_i$, which effectively penalizes predictions that remain unchanged despite content modifications.

% Here, we derive the relaxation weight by penalizing content-independent predictions as follows: $\omega_\text{relaxation} = 1-\gamma^{content}_i$

% \subsection{Relaxation for Collapse}\label{sec:method-relaxation}
% SICL assumes that a model effectively disentangles style and content. However, during continuous adaptation in TTA, model often falls into a collapsed state where it overly attends to the style rather than content during its predictions, hence making the style invariance term unreliable. Thus, we introduce a relaxation weight $\omega_\text{relaxation}$ that penalizes content-independent predictions that overly attend on the \textit{style}.
% To identify the content-independent predictions, we calculate the content invariance ratio $\gamma^{content}_i$ which quantifies the invariance of predictions with respect to content distortion. Specifically, we calculate the content invariance ratio $\gamma^{content}_i$ as follows:
% \[
% \gamma^{content}_i = \frac{1}{N} \sum_{j=1}^{N} \mathbb{I}\left( \hat{y}_i = \hat{y}_{i,j}'' \right)
% \]
% where $\hat{y}_{i,j}''$ denotes the predictions of content-distorted sample $\mathbf{x}_i''$. To simulate content distortion, we utilized the \textit{Content Perturbation} from Section \ref{sec:ideal_ensemble}. Here, we derive the relaxation weight $\omega_\text{relaxation}$ by penalizing content-independent predictions through the subtraction of $\gamma^{content}_i$ from 1. Our final calibrated prediction confidence of $\mathbf{x}_i$ is calculated as follows:
% \[
%     p_{\text{calibrated}}(y_i) = \omega_\text{relaxation}\cdot\gamma^{style}_i = (1-\gamma^{content}_i)\cdot\gamma^{style}_i
% \]



%If the predictions tend to remain invariant after content distortion, this implies that the model is focusing more on style rather than content in making its predictions.

% We first obtain the whitened embeddings (content-specific embedding) as follows: $\mathbf{f}_{\text{white}} = \frac{\mathbf{f}_i - \mu_i}{\sigma_i + \epsilon}$. Next, we add gaussian noise to perturb its content; concretely as follows:
% \[
%     \mathbf{f}_{\text{content-perturb}} = \sigma_i \cdot (\mathbf{f}_{\text{white}} + \mathbf{\epsilon}) + \mu_i 
% \]

% where, $ \mathbf{\epsilon}$ is the gaussian noise \(\epsilon_\sigma  \sim \mathcal{N}(0, \sigma^{\text{white}}_i \cdot I)\). In essence, we're applying standard gaussian noise scaled to the channel-wise standard deviations of the whitened features.



% \subsection{Relaxation for Collapse}\label{sec:method-relaxation}
% Our style-invariance framework assumes that a model effectively disentangles style and content. However, during continuous adaptation in TTA, model often falls into a collapsed state where it overly attends to the style rather than content during its predictions, hence making the style invaraince term unreliable. Thus, we introduce a relaxation term that penalizes predictions that overly attend on the "style".

% Specifically, we calculate the content perturbation consistency ratio $\gamma^{content}_i$, which quantifies the invaraince of predictions with respect to content perturbations. If the predictions tend to remain invaraint after content perturbations, this implies that the model is focusing more on style rather than content in making its predictions. We first obtain the whitened embeddings (content-specific embedding) as follows: $\mathbf{f}_{\text{white}} = \frac{\mathbf{f}_i - \mu_i}{\sigma_i + \epsilon}$. Next, we add gaussian noise to perturb its content; concretely as follows:
% \[
%     \mathbf{f}_{\text{content-perturb}} = \sigma_i \cdot (\mathbf{f}_{\text{white}} + \mathbf{\epsilon}) + \mu_i 
% \]

% where, $ \mathbf{\epsilon}$ is the gaussian noise \(\epsilon_\sigma  \sim \mathcal{N}(0, \sigma^{\text{white}}_i \cdot I)\). In essence, we're applying standard gaussian noise scaled to the channel-wise standard deviations of the whitened features.


% Our framework assumes that the model could capture semantic contents. However, during continuous adaptation across diverse streams, the model may fall into collapsed state where the model fails to capture semantic content and instead relies on style features. To maintain robust calibration performance in such scenarios, we introduce a relaxation term to 




% we introduce a relaxation term to reduce overconfidence. Specifically, we model collapsed degree by variance among maximum class probability (MCP) of style variants, basaed on the intuition that in a collapsed state, the model becomes overly sensitive to style features, leading to significant fluctuations in MCP across candidate style variants. Concretely, we leverage to compute a relaxation weight \( \omega \) for the final confidence. Specifically, given a sample \( \mathbf{x}_i \) with \( N \) style variants, we denote MCP for each style variant \( j \) as \( \phi_{i,j} = \max_{c} \left( \frac{\exp(z_{i,j,c})}{\sum_{k=1}^{C} \exp(z_{i,j,k})} \right) \) where \( z_{i,j,c} \) represents the logit for class \( c \).
% Then, the \( \omega \) for batch \( b \) is calculated as follows:

% \begin{equation}
%  \omega = 1 - \left( \frac{\overline{\sigma^2}_{b}}{\sigma^2_{\text{max}}} \right)^n, \text{where} \quad \overline{\sigma^2}_{b} = \frac{1}{B} \sum_{i=1}^{B} \sigma^2(\phi_{i,1:N}).
% \end{equation}
% Here, \( \sigma^2 \) denotes the variance,  \( B \) denotes the batch size, \( n \) is a hyperparameter for sensitivity, and \( \sigma^2_{\text{max}}\) is the theoretical maximum variance where \( \phi \) values are distributed across their widest possible range. 

% Finally, we obtain the final prediction confidence for each sample \( \mathbf{x}_{i} \) by applying this relaxation weight \( \omega \) to the prediction consistency \( \gamma_i \).









==> sec/6_experiments.tex <==
\section{Experiments}\label{sec:experiments}
% In this section, we present the experimental setup along with both quantitative and qualitative results. Additional details on the experimental configurations are provided in the Appendix. %\ref{sec:appendix_results}, 
In this section, we present the experimental setup along with both quantitative and qualitative results. Additional details on the experimental configurations and outcomes are provided in the Appendix. %\ref{sec:appendix_results}, \ref{sec:appendix_exp_details}.
\subsection{Experimental Setup}\label{sec:exp_setup}
%\noindent\textbf{Datasets.}
\paragraph{Datasets \& Models.}
We evaluate SICL on three widely-used benchmarks: CIFAR10-C, CIFAR100-C, ImageNet-C~\cite{cifarc}. These datasets simulate diverse types of distribution shifts, from simple noise to complete domain shifts, commonly encountered in real-world scenarios. CIFAR10-C and CIFAR100-C contains 15 different synthetic corruptions with five levels of corruption, where we adopt the highest severity level 5 for our experiments. CIFAR10-C/CIFAR100-C contain 10/100 classes, with 10000/1000 samples, respectively. ImageNet-C
dataset contain 50,000 test samples with 1000 classes. For backbone architecture, We use pretrained ResNet-50, 101~\cite{resnet} and ViT~\cite{dosovitskiy2020image} (ViT-Small for CIFAR10/100-C, and ViT-Base for ImageNet-C). For Vision Transformers, we implement our style perturbation approach on the patch embedding space by utilizing the patch-wise mean and standard deviation as a style statistics, following intuitions from TFS-ViT~\cite{noori2024tfs}.

% We evaluate SICL on four widely-used benchmarks: CIFAR10-C~\cite{cifarc}, CIFAR100-C~\cite{cifarc}, OfficeHome~\cite{Venkateswara_2017_CVPR} and Office-31~\cite{saenko2010adapting}. These datasets simulate diverse types of distribution shifts, from simple noise to complete domain shifts, commonly encounted in real-world scenarios. CIFAR10-C and CIFAR100-C contains 15 different synthetic corruptions with five levels of corruption, where we adopt level 5 for our experiments. CIFAR10-C/CIFAR100-C contain 10/100 classes, with 10000/1000 samples, respectively. OfficeHome and Office-31 are datasets commonly used for Unsupervised Domain Adaptation (UDA). OfficeHome consists of 4 domains - art, clipart, product and realworld, with 15,588 images with 65 classes. Office31 consists of 3 domains - amazon, dslr and webcam, including 6,712 images with 31 classes. Following prior study~\cite{sotta}, we use pretrained ResNet18~\cite{resnet} as adapatation target.
% We evaluate SICL on four widely-used benchmarks: CIFAR-10-C, CIFAR-100-C, Office-Home, and Office-31. These datasets simulate various types of distribution shifts, such as corruption, noise and domain, commonly encountered in real-world scenarios. CIFAR10-C and CIFAR100-C include 10, 100 classes, containing 10,000, 10,000 test samples, respectively. Both datasets consist of 15 corruption types of five severity levels, with level 5 used in our experiments. OfficeHome~\cite{Venkateswara_2017_CVPR} is consisted of 4 domains: art, clipart, product, and real, which includes 15,588 images and 65 classes. Office-31~\cite{saenko2010adapting} is cossist of 3 domains: amazon, dslr, and webcam which includes 6,712 images and 31 classes. We use a pre-trained ResNet-18 model, following previous TTA works.

%\paragraph{Implementation Details.}

\paragraph{Scenario.}
To account for diverse distributions in real-world test streams, we define the following two test stream distributions. 
\begin{itemize}
    \item \textbf{Benign}: Assuming a fixed test distribution where a single corruption type (\textit{e.g.} Gaussian noise) is fixed throughout test, where samples arrive in an \textit{i.i.d.} manner.
    % \item \textbf{Noisy}: Assuming a far-distribution shift~\cite{sotta}, where out-of-distribution samples are randomly injected in the \textbf{Benign} test distribution. For our experiments, we utilize MNIST data~\cite{mu2019mnist} to simulate OOD noise. 
    \item \textbf{Dynamic}: Assuming a realistic test distribution, where corruption type has temporal correlation (\textit{i.e.} corruption types arriving at varying lengths). We adopt Dirichlet function to simulate temporal correlation of corruptions  (\textit{e.g. Gaussian noise $\rightarrow$ Shot noise $\rightarrow$ Defocus blur ...}).
\end{itemize}

% First, a \textit{Benign} scenario where the corruption type(\textit{e.g.} Gaussian noise) is fixed throughout the test distribution.  Second, a \textit{Noisy} scenario, which incorporates out-of-distribution (OOD) noise into the stream. We utilize MNIST data~\cite{deng2012mnist} as OOD noise to simulate far-distribution shift, following the setup of SoTTA~\cite{sotta}. Finally, a 



% Finally, a \textit{Dynamic} scenario constitutes various corruption types or domains in a non-i.i.d. manner to simulate dynamic test stream by adopting Dirichlet distribution .These scenarios are designed to reflect a range of distributional shifts that models are likely to face in practical settings.


% \noindent\textbf{Implementation Details}
% For fair comparisons, we integrate SICL into five existing TTA methods, including TENT~\cite{wang2021tent}, EATA~\cite{eata}, SAR~\cite{niu2022towards}, RoTTA~\cite{yuan2023robust}, and SoTTA~\cite{gong2023sotta}. The SICL framework operates in a plug-and-play manner, meaning it requires no additional training or modifications to the base TTA models. During evaluation, we set the number of style perturbations per sample to \( N = 10 \) and apply a Gaussian noise parameter \(\delta\) to control perturbation magnitude, ensuring consistent generation of realistic style variants. All experiments are conducted on NVIDIA V100 GPUs, with PyTorch as the primary deep learning framework.

% \paragraph{TTA Methods.}
% To demonstrate the effectiveness of our method, we evaluate 5 representative TTA methods. For Entropy-based methods, TENT~\cite{tent}, which updates batch normalization through entropy minimization, and EATA~\cite{eata}, which combines entropy thresholding with anti-forgetting regularization. For robust optimization, SAR~\cite{sar} and SoTTA~\cite{sotta} which utilze sharpness-aware minimization while SoTTA also employs high-confidence uniform sampling for noisy streams. Lastly, RoTTA~\cite{rotta} leverages balanced sampling with robust batch normalization, accounting for timeliness and uncertainty.

% Entropy TS updates the temperature based on entropy minimization during adaptation. 


\paragraph{Baselines.}
We evaluate SICL upon 5 different TTA methods - namely TENT~\cite{tent}, EATA~\cite{eata}, SAR~\cite{sar}, RoTTA~\cite{rotta} and SoTTA~\cite{sotta}. For ViT backbones, we consider TENT-LN and SAR-LN, both a variants which updates the affine parameters of the layer normalization layers instead of batch normalization. For calibration baselines, we consider 4 representative methods applicable during TTA scenario. Vanilla TS~\cite{guo2017calibration} applies a fixed temperature learned from the validation dataset of source to calibrate confidence. MC Dropout~\cite{gal2016dropout} uses stochastic dropout at inference to create an ensemble of predictions, capturing uncertainty through averaging. TransCal~\cite{wang2020transferable} estimates target calibration error with the source distribution by introducing importance weighting. Lastly, PseudoCal~\cite{hupseudo} trains the temperature parameter with pseudo-data generated by Mixup~\cite{zhang2018mixup}. Note that, other than MC Dropout, PseudoCal and SICL, we relax the constraints of TTA; allowing the usage of source data for calibrations.

% Entropy TS updates temperature parameter with the entropy minimization objective function in an adaptive manner.

\definecolor{verylightblue}{RGB}{235, 245, 255} % Very light blue for "o"
\definecolor{verylightred}{RGB}{255, 235, 235} % Very light red for "x"

%\input{ICCV2025-Author-Kit-Feb/tables/full_table}


% \begin{table*}[t]
% \centering
% \caption{Expected Calibration Error (ECE) (\%) of uncertainty estimation on CIFAR10-C, CIFAR100-C, and ImageNet-C across five TTA methods under benign test streams. \textbf{Bold} numbers represent the lowest error.}
% \label{tab:main_results_benign}
% \resizebox{.9\textwidth}{!}{%
% \begin{tabular}{llccccccccccccc}
% \toprule
% \multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Method}} 
% & \multicolumn{5}{c}{\textbf{ResNet-50}} 
% & \multicolumn{5}{c}{\textbf{ResNet-101}} 
% & \multicolumn{2}{c}{\textbf{ViT}} 
% & \multicolumn{1}{c}{} \\
% \cmidrule(lr){3-7}\cmidrule(lr){8-12}\cmidrule(lr){13-14}
% & 
% & \textbf{TENT} 
% & \textbf{EATA} 
% & \textbf{SAR} 
% & \textbf{RoTTA} 
% & \textbf{SoTTA} 
% & \textbf{TENT} 
% & \textbf{EATA} 
% & \textbf{SAR} 
% & \textbf{RoTTA} 
% & \textbf{SoTTA} 
% & \textbf{TENT} 
% & \textbf{SAR} 
% & \multicolumn{1}{c}{Avg.} \\
% \midrule

% \multirow{6}{*}{\textbf{CIFAR10-C}}
% & Vanilla TS  & 22.7 & 22.3 & 22.2 & 22.9 & 22.8 & 32.0 & 21.2 & 21.8 & 21.7 & 21.8 & 17.2 & 15.2 & 21.9 \\
% & MC Dropout  & 16.3 & 11.1 & 10.2 & 10.0 & 10.4 & 25.9 & 10.2 & 10.1 & 9.2 & 10.2 & 22.1 & 19.3 & 13.8 \\
% & TransCal    & 56.7 & 56.2 & 56.9 & 11.0 & 56.1 & 48.0 & 57.0 & 57.0 & 52.0 & 56.9 & 26.7 & 26.5 & 44.8 \\
% & PseudoCal   & 9.4  & 7.8  & \textbf{5.2}  & 7.9  & 8.4  & 18.4  & 7.9  & \textbf{5.4}  & 9.0  & 8.6  & 34.9  & 33.6  & 13.9 \\
% & \cellcolor{verylightblue}\textbf{SICL (Ours)} & \cellcolor{verylightblue}\textbf{6.4}  & \cellcolor{verylightblue}\textbf{6.9}  & \cellcolor{verylightblue}7.5  & \cellcolor{verylightblue}\textbf{7.1}  & \cellcolor{verylightblue}\textbf{7.5}  & \cellcolor{verylightblue}\textbf{6.6}  & \cellcolor{verylightblue}\textbf{7.6}  & \cellcolor{verylightblue}8.0  & \cellcolor{verylightblue}\textbf{7.3}  & \cellcolor{verylightblue}\textbf{8.0}  & \cellcolor{verylightblue}\textbf{8.4}  & \cellcolor{verylightblue}\textbf{8.7}  & \cellcolor{verylightblue} \textbf{7.7} \\
% \cmidrule(lr){2-15}
% & Acc & 77.1 & 75.7 & 77.5 & 74.9 & 77.0 & 68.4 & 76.8 & 78.2 & 76.3 & 78.2 & 53.0 & 53.0 &  \\
% \midrule
% \multirow{6}{*}{\textbf{CIFAR100-C}}
% & Vanilla TS  & 9.6 & 22.7 & 7.0 & 12.5 & 6.0 & 13.8 & 36.4 & 9.3 & 9.6 & 7.9 & 18.2 & 17.2 & 13.8 \\
% & MC Dropout  & 13.5 & 16.0 & 8.7 & 13.6 & 8.4 & 20.0 & 12.7 & 9.2 & 8.6 & 8.5 & 19.9 & 18.2 & 12.8 \\
% & TransCal    & 50.0 & 27.5 & 8.1 & 36.6 & 12.0 & 18.7 & 13.2 & 56.3 & 11.7 & 23.8 & 23.0 & 22.5 & 22.6 \\
% & PseudoCal   & \textbf{7.4} & 7.3 & 8.7 & 8.1 & 9.0 & 10.8 & 7.4 & \textbf{8.4} & 7.5 & 6.6 & 34.9 & 33.6 & 13.5 \\
% & \cellcolor{verylightblue}\textbf{SICL (Ours)} & \cellcolor{verylightblue}7.5 & \cellcolor{verylightblue}\textbf{6.6} &\cellcolor{verylightblue} \textbf{7.9} & \cellcolor{verylightblue}\textbf{6.2} & \cellcolor{verylightblue}\textbf{7.7} & \cellcolor{verylightblue}\textbf{5.4} & \cellcolor{verylightblue}\textbf{5.6} & \cellcolor{verylightblue}6.6 & \cellcolor{verylightblue}\textbf{5.3} & \cellcolor{verylightblue}\textbf{6.6} & \cellcolor{verylightblue}\textbf{8.4} & \cellcolor{verylightblue}\textbf{8.7} & \cellcolor{verylightblue}\textbf{6.8} \\
% \cmidrule(lr){2-15}
% & Acc & 52.7 & 33.1 & 54.2 & 49.7 & 51.1 & 44.1 & 19.4 & 55.8 & 51.6 & 52.5 & 50.8 & 50.9 &  \\
% \midrule
% \multirow{6}{*}{\textbf{ImageNet-C}}
% & Vanilla TS  & 23.9 & 23.2 & 13.4 & 13.4 & 13.2 & 20.7 & 36.4 & 15.7 & 13.7 & 15.7 & 19.8 & 11.9 & 17.4 \\
% & MC Dropout  & 11.0 & 13.7 & 15.2 & 14.6 & 16.8 & 12.0 & 12.7 & 13.6 & 11.8 & 12.6 & 28.9 & 28.8 & 16.7 \\
% & TransCal    & 14.5 & 8.6 & \textbf{8.1} & 9.2 & 9.8 & \textbf{11.0} & 34.3 & 19.2 & 10.6 & 11.1 & 40.5 & 41.8 & 19.6 \\
% & PseudoCal   & 14.1 & 8.5 & 14.9 & 13.7 & 14.9 & 14.0 & 11.6 & 14.7 & 12.9 & 14.8 & 19.0 & 17.4 & 14.8 \\
% & \cellcolor{verylightblue}\textbf{SICL (Ours)} & \cellcolor{verylightblue}\textbf{10.0} & \cellcolor{verylightblue}\textbf{7.4} & \cellcolor{verylightblue}9.1 & \cellcolor{verylightblue}\textbf{7.2} & \cellcolor{verylightblue}\textbf{8.4} & \cellcolor{verylightblue}13.6 & \cellcolor{verylightblue}\textbf{9.6} & \cellcolor{verylightblue}\textbf{12.4} & \cellcolor{verylightblue}\textbf{9.2} & \cellcolor{verylightblue}\textbf{10.9} & \cellcolor{verylightblue} \textbf{15.5} & \cellcolor{verylightblue} \textbf{11.1} & \cellcolor{verylightblue} \textbf{10.7} \\
% \cmidrule(lr){2-15}
% & Acc & 36.3 & 21.0 & 33.2 & 31.1 & 29.0 & 40.0 & 22.9 & 36.3 & 32.7 & 30.5 & 40.7 & 49.0 &  \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}


% \begin{table*}[t]
% \centering
% \caption{Expected Calibration Error (ECE) (\%) of uncertainty estimation on CIFAR-10C, CIFAR-100C, and ImageNet-C across five TTA methods under dynamic test streams. \textbf{Bold} numbers represent the lowest error.}
% \label{tab:main_results_dynamic}
% \resizebox{.9\textwidth}{!}{%
% \begin{tabular}{llccccccccccccc}
% \toprule
% \multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Method}} 
% & \multicolumn{5}{c}{\textbf{ResNet-50}} 
% & \multicolumn{5}{c}{\textbf{ResNet-101}} 
% & \multicolumn{2}{c}{\textbf{ViT}} 
% & \multicolumn{1}{c}{} \\
% \cmidrule(lr){3-7}\cmidrule(lr){8-12}\cmidrule(lr){13-14}
% & 
% & \textbf{TENT} 
% & \textbf{EATA} 
% & \textbf{SAR} 
% & \textbf{RoTTA} 
% & \textbf{SoTTA} 
% & \textbf{TENT} 
% & \textbf{EATA} 
% & \textbf{SAR} 
% & \textbf{RoTTA} 
% & \textbf{SoTTA} 
% & \textbf{TENT} 
% & \textbf{SAR} 
% & \multicolumn{1}{c}{Avg.} \\
% \midrule

% \multirow{7}{*}{\textbf{CIFAR10-C}}
% & Vanilla TS  & 12.9 & 18.4 & 23.7 & 21.3 & 23.6 & 11.4 & 18.5 & 23.7 & 21.6 & 23.7 & 11.2 & 10.1 & 18.3 \\
% & MC Dropout  & 15.4 & 18.7 & 10.4 & 15.9 & 10.4 & 17.8 & 19.5 & 10.4 & 14.3 & 10.4 & 23.8 & 24.0 & 15.9 \\
% & TransCal    & 56.4 & 47.3 & 57.0 & 43.8 & 56.9 & 53.1 & 46.2 & 57.2 & 46.2 & 57.2 & 28.1 & 27.7 & 48.1 \\
% & PseudoCal   & 17.1 & 7.5  & 12.4 & 14.1 & 12.5 & 23.4 & 7.3 & 12.5 & 14.4 & 12.5 & 25.6 & 25.5 & 15.4 \\
% & \cellcolor{verylightblue}\textbf{SICL (Ours)} & \cellcolor{verylightblue}\textbf{5.9}  & \cellcolor{verylightblue}\textbf{5.8}  & \cellcolor{verylightblue}\textbf{6.9}  &\cellcolor{verylightblue} \textbf{6.2}  & \cellcolor{verylightblue}\textbf{6.9}  & \cellcolor{verylightblue}\textbf{6.6}  & \cellcolor{verylightblue}\textbf{6.3}  & \cellcolor{verylightblue}\textbf{7.3}  & \cellcolor{verylightblue}\textbf{7.1}  & \cellcolor{verylightblue}\textbf{7.4}  & \cellcolor{verylightblue}\textbf{7.8}  & \cellcolor{verylightblue}\textbf{7.4}  & \cellcolor{verylightblue}\textbf{7.1}  \\
% \cmidrule(lr){2-15}
% & Acc & 77.2 & 68.6 & 77.6 & 67.9 & 77.6 & 74.3 & 70.2 & 78.3 & 69.8 & 78.3 & 56.8 & 56.4 &  \\\midrule
% %\midrule

% \multirow{7}{*}{\textbf{CIFAR100-C}}
% & Vanilla TS  & 51.7 & 55.3 & 46.6 & 53.8 & 48.3 & 60.5 & 54.4 & 45.2 & 53.0 & 47.1 & 9.3  & 7.8  & 44.4 \\
% & MC Dropout  & 11.1 & 19.4 & 9.5  & 16.3 & 10.0 & 18.3 & 22.3 & 6.6  & 10.4 & 6.8  & 8.7  & 9.1  & 12.4 \\
% & TransCal    & 43.6 & 34.5 & 48.4 & 29.8 & 46.4 & 33.4 & 35.9 & 50.0 & 32.1 & 47.8 & 23.3 & 22.7 & 37.3 \\
% & PseudoCal   & 21.2 & 9.7  & 16.3 & 19.4 & 16.3 & 30.6 & 8.9 & 15.8 & 18.2 & 15.0 & 31.0 & 31.6 & 19.5 \\
% & \cellcolor{verylightblue}\textbf{SICL (Ours)} & \cellcolor{verylightblue}\textbf{6.6}  & \cellcolor{verylightblue}\textbf{4.4}  & \cellcolor{verylightblue}\textbf{7.8}  & \cellcolor{verylightblue}\textbf{3.8}  & \cellcolor{verylightblue}\textbf{8.0}  & \cellcolor{verylightblue}\textbf{4.6}  & \cellcolor{verylightblue}\textbf{4.5}  & \cellcolor{verylightblue}\textbf{6.6}  & \cellcolor{verylightblue}\textbf{3.5}  & \cellcolor{verylightblue}\textbf{6.5}  & \cellcolor{verylightblue}\textbf{4.5}  & \cellcolor{verylightblue}\textbf{4.7}  & \cellcolor{verylightblue}\textbf{5.5}  \\
% \cmidrule(lr){2-15}
% & Acc & 45.7 & 43.7 & 50.6 & 36.7 & 48.6 & 36.9 & 44.7 & 52.2 & 38.8 & 50.0 & 28.3 & 27.6 &  \\\midrule
% %\midrule

% \multirow{7}{*}{\textbf{ImageNet-C}}
% & Vanilla TS  & 23.9 & 14.2 & 13.4 & 13.4 & 13.2 & 20.7 & 9.5 & 15.7 & 13.7 & 15.7 & 19.8 & 11.9 & 15.4 \\
% & MC Dropout  & 12.1 & 12.4 & 6.8  & 9.2 & 6.7  & 17.9 & 15.9  & 14.1  & 18.4  & 7.9  & 28.9 & 28.8 & 14.9 \\
% & TransCal    & 14.5 & 29.5 & \textbf{8.1}  & 9.2  & 8.0  & \textbf{11.0} & 32.2 & 9.2  & 10.6 & 9.1  & 40.5 & 41.8 & 18.6 \\
% & PseudoCal   & 10.7 & 8.1 & 15.0  & 13.5  & 14.9  & 11.5 & 8.7  & \textbf{7.2}  & 9.0 & 7.1  & 13.5  & 11.0  & 10.9 \\
% & \cellcolor{verylightblue}\textbf{SICL (Ours)} & \cellcolor{verylightblue}\textbf{8.9}  & \cellcolor{verylightblue}\textbf{7.7}  & \cellcolor{verylightblue}8.7  & \cellcolor{verylightblue}\textbf{6.5}  & \cellcolor{verylightblue}\textbf{6.3}  & \cellcolor{verylightblue}12.4  & \cellcolor{verylightblue}\textbf{8.5}  & \cellcolor{verylightblue}8.3  & \cellcolor{verylightblue}\textbf{8.4}  & \cellcolor{verylightblue}\textbf{6.9}  & \cellcolor{verylightblue}\textbf{10.1}  & \cellcolor{verylightblue}\textbf{8.0}  & \cellcolor{verylightblue}\textbf{8.4}  \\
% \cmidrule(lr){2-15}
% & Acc & 37.5 & 31.9 & 36.7 & 34.1 & 31.2 & 33.8 & 34.0 & 32.4 & 31.6 & 33.2 & 44.1 & 45.2 &  \\\bottomrule
% %\bottomrule
% \end{tabular}%
% }
% \end{table*}
%\vspace{-10pt}

\input{wacv-2026-author-kit-template/tables/main_table}




\subsection{Main Results}\label{sec:main_results}

In this section, we present our main experimental results, highlighting the effectiveness of SICL across various TTA scenarios. All experiments in this subsection were conducted three times, with results averaged to ensure fair comparisons. Also, we reported the average results across 15 corruption types for all experiments.  Table \ref{tab:main_results} shows the results on three datasets with three model architecture under benign, and dynamic stream. SICL achieved state-of-the-art calibration performance in almost all settings (63/72). On average across all datasets, scenarios, model architectures, and TTA methods, SICL outperforms baselines by 13.0\%p. In particular, it outperforms baselines by an average of 15.6\%p in the Dynamic Stream and by an average of 10.4\%p in the benign Stream, which demonstrates the superiority of SICL in situations where the test distribution is not fixed but changes dynamically.


% Overall, it is challenging to identify consistent trends in calibration performance due to the wide variety of distribution shifts present in datasets within various test streams, and the characteristics of online models with applied TTA methods. Nevertheless, the fact that SICL consistently achieves the lowest calibration error demonstrates its robustness in handling the diverse scenarios faced by deployed models during test time.

% SICL achieves lowest calibration error across all scenarios and TTA methods even without additional training for temperature. Specifically, it outperforms other baselines in handling dynamic and noisy test streams, where traditional calibration methods often struggle due to the evolving and unpredictable nature of data distributions in TTA. By leveraging style invariance, SICL provides robust calibration that adapts effectively to real-world shifts, maintaining reliability without additional training or accuracy trade-offs. 



\subsection{Qualitative Analysis}\label{sec:analysis}
\input{figs/analysis}
\input{wacv-2026-author-kit-template/figs/ablation}In our earlier discussion (Section \ref{sec:motivation}), we examined the conditions for an ideal ensemble candidate representation, highlighting the importance of preserving the content of the original sample while simulating various style changes. Based on these conditions, we conducted an analysis to assess how qualitatively superior representations generated by our style perturbation are compared to conventional style-shift methods represented by MixStyle~\cite{zhou2021domain}. First, we measure the degree of content preservation by utilizing the average \textit{ContentVariance} defined in Section \ref{sec:content_analysis}. In Figure ~\ref{Fig:analysis} (a), we could see that our \textit{Style Perturbation} shows lower mean distance difference than MixStyle regardless of corruption types. Second, we measured style variance by repurposing the style reconstruction loss~\cite{johnson2016perceptual} to evaluate how well our method simulates diverse styles. For each sample $\mathbf{z}_i$ and its style-variant $\mathbf{z}^{s\prime}_i$, we calculate \textit{StyleVariance} as follows:
% For each target sample $\mathbf{x}_i$ and its style-variant $\mathbf{x'}_i$, we calculate Style Variance as the squared Frobenius norm of the difference between the Gram matrices ($G$) of the original and style-shifted samples:
\[
 \textit{StyleVariance}(\mathbf{z}_i, \mathbf{z}^{s\prime}_i) =  \|G(\mathbf{z}_i) - G(\mathbf{z}^{s\prime}_i)\|_F^2 
\]
where $G$ denotes the Gram Matrix~\cite{Gatys_2016_CVPR} that encodes style information. In Figure~\ref{Fig:analysis} (b), we plot the average \textit{StyleVariance} of each sample in the CIFAR10-C dataset with its 20 style-variants. It can be seen that the style-perturbed embeddings from SICL exhibit a higher \textit{StyleVariance} across all corruption types than Dropout or MixStyle-generated embeddings. Thus, we find our style perturbation to generate proper candidate embeddings that 1) maintain content integrity while 2) exhibiting higher style diversity, enabling reliable and accurate prediction of model's confidence. In the case of MixStyle, it creates a new style by mixing the style statistics of two samples from the available target set (in the TTA situation, this is the online test batch). This is dependent on the composition of the input batch and cannot simulate as diverse a variation in the style space as \textit{Style Perturbation}, which leads to deficiencies in the quality aspect of style variant representation.


% Similar with the motivational analysis (Section \ref{sec:motivation}), we compare embeddings generated from MixStyle~\cite{zhou2021domain} and our style perturbation to evaluate the quality of style-shifted ensemble candidate representation. In Figure ~\ref{Fig:analysis} (a), we could see that our style perturbation shows lower mean distance difference than MixStyle. Furthermore, we visualize the variability of the generated embeddings $\mathbf{z}_i$ on Figure~\ref{Fig:analysis} (b). Here, we plot the mean variance of candidate embeddings of each sample in the CIFAR-10C dataset. It can be seen that the style-perturbed embeddings from SICL exhibit a higher variability across most (14/15) corruption types than MixStyle-generated embeddings. Thus, we find our style perturbation to generate proper candidate embeddings that 1) maintain content integrity while 2) exhibiting higher diversity, enabling reliable and accurate prediction of model's confidence. In the case of MixStyle, it creates a new style by mixing the style statistics of two samples from the available target set (in the TTA situation, this is the online test batch). This is dependent on the composition of the input batch and cannot simulate as diverse a variation in the Style Space as Style Perturbation, which leads to deficiencies in the quality aspect of style variant representation.


\subsection{Ablation Studies}\label{sec:ablation}
% \begin{table}[t]
% \centering
% \caption{Expected Calibration Error (ECE) (\%) of  style variation methods on CIFAR 10-C across TTA methods. \textbf{Bold} numbers represent the lowest error.}
% \label{tab:style_variation}
% \scriptsize
% \renewcommand{\arraystretch}{1.2} % Adjust row height for readability
% \setlength{\tabcolsep}{4pt} % Adjust column spacing for single-column fit
% \begin{tabular}{lcccccc}
% \toprule
% \multirow{2}{*}{\centering \makecell{Style Variation\\Method}} & \multicolumn{5}{c}{TTA Method} \\ \cline{2-6} \addlinespace[0.3em]
% & TENT & EATA & SAR & RoTTA & SoTTA & Avg. ($\downarrow$) \\ \midrule
% Style Interpolation & 11.27 & 12.79 & 12.48 & 13.76 & 12.82 & 12.57 \\
% MixStyle  & 8.53 & 8.01 & 8.51 & 9.94 & 8.76 & 8.75 \\
% Style Perturbation ($\sigma$) & 8.51 & 7.85 & 8.37 &11.18 & 8.59 & 8.98 \\
% Style Perturbation ($\mu$) & 5.31 & 3.58 & 4.84 & 6.91 & 4.95 & 5.16 \\
% Style Perturbation ($\mu, \sigma$) & \textbf{2.89} & \textbf{3.33} & \textbf{3.30} &  \textbf{5.22} & \textbf{2.42} & \textbf{3.32} \\ 
% \bottomrule
% \end{tabular}
% \end{table}



% \begin{figure}[htbp]
%     \centering
%     %\includegraphics[width=\columnwidth]{wacv-2026-author-kit-template/figs/raw_figs/ablation_final.pdf}
%     \includegraphics[width=\textwidth]{wacv-2026-author-kit-template/figs/raw_figs/ablation_final.pdf}
%     \vspace{-20pt}
%     \caption{Ablation results on (a) individual components of SICL, and (c) upon the number of variants $N$ across baseline TTA algorithms.}
%     \label{fig:ablation_studies}
%     \vspace{-10pt}
% \end{figure}
%\subsection{Ablation for style variation}\label{sec:ablation_stylevariantion}
On the subsequent paragraphs, we conduct ablative studies on (1) effect of style variations by progressively removing each components, (2) effect of relaxation weight, and (3) effect of the number of variations generated ($N$). Note that all the ablative experiments were conducted upon CIFAR-100-C, with ResNet-50 backbone.


\paragraph{Ablation on style variation.}
We conduct a comprehensive ablation study to evaluate SICL against existing style variation methods and analyze the contribution of individual components. We mainly compare our \textit{Style Perturbation} with MixStyle~\cite{zhou2021domain}, which generates novel styles through pairwise mixing of feature-level style statistics within a batch. Additionally, we examine the individual impact of style components through: isolated perturbation of the fine-grained style attribute $\sigma$, and isolated perturbation of the coarse-grained style attribute $\mu$. The comparative results are presented in Figure~\ref{fig:ablation_studies} (a). It can be seen that our \textit{Style Perturbation} method consistently achieves superior performance across all TTA frameworks, validating its robustness and versatility. Notably, our analysis reveals that the influence of the coarse style attribute $\mu$ is greater than that of the fine style attribute $\sigma$, which aligns with prior findings~\cite{huang2017arbitrary}. Furthermore, the optimal calibration performance is achieved when combining both $\mu$ and $\sigma$, indicating their complementary roles in effective style variation.

% \paragraph{Ablation on style variation.}
% We conduct a comprehensive ablation study to evaluate SICL against existing style variation methods and analyze the contribution of individual components. Our evaluation encompasses two baseline approaches from the literature: (1) MixStyle~\cite{zhou2021domain}, which generates novel styles through pairwise mixing of style statistics within a batch, and (2) Style interpolation, which synthesizes new styles via batch-wise weighted averaging of style statistics. Additionally, we examine the individual impact of style components through: (3) isolated perturbation of the fine-grained style attribute $\sigma$, and (4) isolated perturbation of the coarse-grained style attribute $\mu$. The comparative results are presented in Figure~\ref{fig:ablation_studies}(a). It can be seen that our style perturbation method consistently achieves superior performance across all TTA frameworks, validating its robustness and versatility. Notably, our analysis reveals that the influence of the coarse style attribute $\mu$ is greater than that of the fine style attribute $\sigma$, particularly in terms of effective perturbation, which aligns with prior findings~\cite{huang2017arbitrary}. Furthermore, the optimal calibration performance is achieved when combining both style attributes, indicating their complementary roles in effective calibration.

% We conduct an ablative study for style variation methods. All methods in this study employ channel-wise mean and standard deviation as style statistics. For MixStyle, a technique used in ~\cite{zhou2021domain}, two samples are selected from the batch, and their style statistics are mixed to generate novel style. In Style Interpolation, a new style is synthesized by taking a weighted average of style statistics across all batch samples. As shown in Table \ref{tab:style_variation}, the results show that Style Perturbation consistently outperforms other methods across different TTA methods, demonstrating its robustness by generating novel candidates which mimic realistic shifts for prediction consistency.  Additionally, the study reveals that the influence of the coarse style attribute \( \mu \) is greater than that of the fine style attribute \( \sigma \), especially in terms of effective perturbation which is consistent with prior study~\cite{huang2017arbitrary}. Notably, combining both style attributes yields the best calibration performance, indicating the complementary role of both attributes.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.95\columnwidth]{figs/raw_figs/hyperparam_sensitivity.pdf}
%     \caption{Hyperparameter sensitivity analysis of SICL on number of style variants $N$.}
%     \label{fig:hyperparameter_sensitivity}
%     \vspace{-5pt}
% \end{figure}

\paragraph{Ablation on relaxation weight.}\label{sec:ablation_relaxation}
We further conduct an ablative study upon the relaxation term. The results are visualized in Figure~\ref{fig:ablation_studies} (b), where SICL denotes the final performance after applying relaxation weight  $\omega_\text{relaxation}$ to style invariance ratio $\gamma^{style}_i$ as a calibrated prediction confidence. It can be seen that $\omega_\text{relaxation}$ brings consistent improvements in uncertainty estimation performance, regardless of the TTA method. Here, we can see that the ECE reduction from relaxation is relatively small in SAR~\cite{sar} and SoTTA~\cite{sotta} compared to other methods, which can be attributed to the fact that these two methods already handle collapse to some extent through robust parameter updates based on Sharpness-Aware Minimization~\cite{foret2020sharpness}.

% Notably, this enhancement is particularly pronounced in TENT~\cite{tent}, which is attributed to its lack of model collapse mitigation mechanisms - strategies to prevent or delay model collapse during adversarial data stream processing, which is present in recent approaches~\cite{eata, sar, rotta, sotta}.


% As shown in Figure \ref{fig:relaxation}, we investigate the impact of the relaxation by measuring the ECE reduction across various TTA methods for various test stream on CIFAR-10C. In general, we observe a reduction in calibration error within dynamic test streams, where diverse corruptions are dynamically introduced, leading to the highest frequency of model collapse. In contrast, for benign and noisy streams—where collapse is less prevalent—the relaxation weight shows minimal impact or even a small increase in calibration error across TTA methods. Overall, these shows that SICL with simple relaxation enables the model to produce robust uncertainty estimates even in cases where collapse frequently occurs without sacrificing a significant performance for scenarios where collapse is less prevalent.

\paragraph{Hyperparameter sensitivity.} 
We show the hyperparameter sensitivity of SICL in Figure~\ref{fig:ablation_studies} (c). The reported expected calibration error is an average upon all data streams (\textit{i.e.} corruption type) and TTA methods. SICL doesn't have any hyperparameters other than the number of style variants. In Figure~\ref{fig:ablation_studies} (c), we plot the calibration performance with respect to number of style variants $N$. We found that SICL demonstrates robustness to the value of $N$ across all TTA methods. Specifically, it achieves sufficiently low calibration error (less than 10\% of ECE) with as few as $N=5$ style variants, and shows a consistent decrease in errors as $N$ increases. For all our experiments including main experiments and additional studies, we choose $N=20$.



% \paragraph{Hyperparameter sensitivity.} 
% We show the hyperparameter sensitivity of SICL in Figure~\ref{fig:hyperparameter_sensitivity} on CIFAR-10C. The reported expected calibration error is an average upon all data streams (\textit{i.e.} corruption type, data stream type). As expected, we find an adequate choice of perturbation magnitude $\delta$ is required - where insufficient noise limits variation while excessive noise may undesirably result in content distortion. However, we find 0.05 to be a good choice - showing robust performance across diverse data streams. In Figure~\ref{fig:hyperparameter_sensitivity} (b), we plot the calibration performance with respect to number of style variants $N$. Notably, we find SICL to be extremely robust to the $N$, reaching a sufficiently low calibration error at even $N=10$, and showing monotonic decrease in errors as $N$ increases. For all our experiments, we choose $N=20$. 


% We evaluated the impact of the number of style variants $N$ and magnitude of perturbation noise $\delta$ on calibration performance. The left plot of Figure \ref{fig:hyperparameter_sensitivity} shows ECE of different TTA methods on CIFAR-10C as the number of style variants $N$ increases. The displayed ECE values are averaged across all test streams. Overall, while increasing $N$ generally reduces calibration error, the ECE remains sufficiently low even at $N=10$. Balancing computational cost, we set $N=20$ for all our experiments. The right plot of Figure \ref{fig:hyperparameters} shows ECE of various test stream on CIFAR-10C as $\delta$ increases. 
% The graph suggests that an appropriate noise range is desirable: excessive noise may distort style attributes, while insufficient noise might limit variation. Notably, this calibration trend appears consistent across different test streams and methods, indicating that the model's response to noise maintains a generally robust pattern.

% , regardless of specific adaptation strategies
% The displayed ECE values are averaged across all TTA baselines. Each test stream exhibits a similar trend across the range of perturbation magnitudes regardless of TTA methods. We use a fixed $\delta$ value of 0.05 for all experiments.
%\noindent\textbf{Impact of Hyperparameter $\delta $.}




==> sec/7_limitation.tex <==
\section{Limitation}\label{sec:limitation}

SICL has the following limitations. First, it assumes that the online model can perform content-driven predictions. This assumption limits its performance on collapsed model. Although calibration on a collapsed model is impractical, and other calibration methods also face the same challenges, SICL addresses this issue by introducing a relaxation term to reduce overconfidence when collapse occurs.
Second, SICL requires multiple forward passes to generate style variants, a common limitation in ensemble-based methods like MC Dropout. However, SICL don't require multiple forward passes on the whole layer, and it also eliminates the need for memory-intensive backward passes.
Despite these limitations, SICL presents fewer constraints compared to other calibration methods, as shown in Table \ref{tab:calibration_comparison}. Moreover, its ability to produce accurate uncertainty estimates across various test streams regardless of adaptation methods makes it an appealing solution for practitioners.

% Moreoveravoiding additional training and backward passes, which would otherwise consume more memory and computation.



%However, unlike MC Dropout, SICL reduces computational demand by only requiring multiple passes on lower layers. Furthermore, it doesn't require any 

% SICL has the following limitations. First, it assumes that the online model can perform content-driven predictions. This assumption limits SICL’s performance on models that have already collapsed, as it relies on the model’s ability to retain content recognition. Although calibration on a malfuctioned model is impractical, and most methods face challenges in such cases, SICL partially addresses this issue by applying a relaxation weight to reduce overconfidence when collapse occurs.
% Second, SICL requires multiple forward passes to generate style variants for measuring prediction consistency, a common limitation in stochastic methods like MC Dropout. However, SICL offers the advantage of not requiring multiple forward passes on the full model, unlike MC Dropout, and it also eliminates the need for memory-intensive backward passes, which are more demanding than forward passes.

% Despite these limitations, SICL presents fewer constraints compared to other calibration methods, as shown in Table \ref{tab:calibration_comparison}. Moreover, its ability to effectively provide robust uncertainty estimates across various test streams in a method-agnostic manner makes it an appealing choice for practitioners.

==> sec/8_conclusion.tex <==

\section{Conclusion}\label{sec:conclusion}
We tackle the critical yet underexplored problem of securing reliable uncertainty estimates in TTA scenarios. To address this challenge, we introduce SICL, the first framework to leverage style invariance for robust uncertainty estimation by providing instance-wise correctness likelihood in real-world test streams. Our comprehensive evaluation demonstrates that SICL consistently outperforms state-of-the-art calibration methods across diverse scenarios and settings while maintaining high practicality. Moreover, we believe our work could inspire further research in both uncertainty estimation for TTA and style-content-driven calibration.


% We tackle the critical yet underexplored problem of securing reliable uncertainty estimates under TTA scenarios. To overcome these difficulties, we presented SICL, a novel framework that firstly leverages style invariance to provide robust instance-wise correctness likelihood estimates in real-world test streams. Our comprehensive evaluation reveals that SICL outperforms state-of-the-art calibration methods in diverse scenarios with high practicality. Moreover, we believe our work could inspire further research in both \textit{calibration for TTA} and \textit{style-content-driven calibration}.

 % Our comprehensive evaluation across 5 TTA methods, 3 benchmarks, 2 scenarios, and 3 architectures reveals that SICL consistently outperforms state-of-the-art calibration methods with high practicality.

% \paragraph{Limitations and future work.}
% SICL has two main limitations. First, it assumes the model performs content-driven predictions, limiting effectiveness on collapsed models. We address this partially through our relaxation term, but future work could develop better collapse-aware mechanisms. Second, similar to other assembly approaches, it requires multiple forward passes to generate style variants. Future research could focus on developing more efficient techniques for style variant generation.

% \section{Limitation}\label{sec:limitation}

% SICL has the following limitations. First, it assumes that the online model can perform content-driven predictions. This assumption limits its performance on collapsed model. Although calibration on a collapsed model is impractical, and other calibration methods also face the same challenges, SICL addresses this issue by introducing a relaxation term to reduce overconfidence when collapse occurs.
% Second, SICL requires multiple forward passes to generate style variants, a common limitation in ensemble-based methods like MC Dropout. However, SICL don't require multiple forward passes on the whole layer, and it also eliminates the need for memory-intensive backward passes.
% Despite these limitations, SICL presents fewer constraints compared to other calibration methods, as shown in Table \ref{tab:calibration_comparison}. Moreover, its ability to produce accurate uncertainty estimates across various test streams regardless of adaptation methods makes it an appealing solution for practitioners.

% \section{Conclusion}\label{sec:conclusion}
% Due to the inherent complexities of TTA where the model and distribution evolving over time, securing reliable uncertainty estimates is difficult. To overcome this challenges, 
% we presented a novel framework that leverages style invariance to provide robust instance-wise correctness likelihood estimates in real-world test stream. By measuring the prediction consistency between original sample and its style variants with realistic shifts, SICL realize reliable test-time adaptation under various practical scenarios. Furthermore, practitioners can easily enhance reliability of deployed model with SICL since it supports seamless integration without any accuracy loss and additional training. Lastly, our findings suggest that relationship between style and content can be effectively used to model uncertainty, offering a promising approach that stimulate further research in this direction.

% While SICL relies on assumptions about model could identify semantic content that may not fully hold universally, experiments show its state-of-the-art calibration performance across diverse test distributions. 



% Furthermore, SICL’s seamless integration with existing adaptation methods makes it a valuable solution for enhancing model reliability in practical, high-stakes environments where trustworthy predictions are essential.

==> tables/full_table.tex <==
% \begin{table*}[t]
% \centering
% \caption{Mean absolute error (MAE) (\%) of the accuracy estimation across various models (ResNet-50, ResNet-101, ViT).}
% \label{tab:styled_table}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llrrrrrrrrrrrrr}
% \toprule
% \multicolumn{2}{c}{} 
% & \multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ResNet-50}} 
% & \multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ResNet-101}} 
% & \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ViT}} 
% & \multicolumn{1}{c}{} \\
% \cmidrule(lr){3-7}\cmidrule(lr){8-12}\cmidrule(lr){13-14}
% \multicolumn{2}{c}{} 
% & \cellcolor[HTML]{EFEFEF}\textbf{TENT} 
% & \cellcolor[HTML]{EFEFEF}\textbf{EATA} 
% & \cellcolor[HTML]{EFEFEF}\textbf{SAR} 
% & \cellcolor[HTML]{EFEFEF}\textbf{ROTTA} 
% & \cellcolor[HTML]{EFEFEF}\textbf{SOTTA} 
% & \cellcolor[HTML]{EFEFEF}\textbf{TENT} 
% & \cellcolor[HTML]{EFEFEF}\textbf{EATA} 
% & \cellcolor[HTML]{EFEFEF}\textbf{SAR} 
% & \cellcolor[HTML]{EFEFEF}\textbf{ROTTA} 
% & \cellcolor[HTML]{EFEFEF}\textbf{SOTTA} 
% & \cellcolor[HTML]{EFEFEF}\textbf{TENT} 
% & \cellcolor[HTML]{EFEFEF}\textbf{SAR} 
% & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}} \\
% \midrule

% \multirow{6}{*}{\textbf{CIFAR-10}} 
% & Vanilla TS  & {\color[HTML]{363A3D}12.9} & {\color[HTML]{363A3D}17.6} & {\color[HTML]{363A3D}23.7} & {\color[HTML]{363A3D}21.3} & {\color[HTML]{363A3D}23.6} & {\color[HTML]{363A3D}11.4} & {\color[HTML]{363A3D}18.5} & {\color[HTML]{363A3D}23.7} & {\color[HTML]{363A3D}21.6} & {\color[HTML]{363A3D}23.7} & {\color[HTML]{363A3D}11.2} & {\color[HTML]{363A3D}10.1} & 18.3 \\
% & MC Dropout  & {\color[HTML]{363A3D}15.4} & {\color[HTML]{363A3D}19.5} & {\color[HTML]{363A3D}10.4} & {\color[HTML]{363A3D}15.9} & {\color[HTML]{363A3D}10.4} & {\color[HTML]{363A3D}17.8} & {\color[HTML]{363A3D}18.8} & {\color[HTML]{363A3D}10.4} & {\color[HTML]{363A3D}14.3} & {\color[HTML]{363A3D}10.4} & {\color[HTML]{363A3D}23.8} & {\color[HTML]{363A3D}24.0} & 15.9 \\
% & TransCal    & {\color[HTML]{363A3D}56.4} & {\color[HTML]{363A3D}46.2} & {\color[HTML]{363A3D}57.0} & {\color[HTML]{363A3D}43.8} & {\color[HTML]{363A3D}56.9} & {\color[HTML]{363A3D}53.1} & {\color[HTML]{363A3D}47.3} & {\color[HTML]{363A3D}57.2} & {\color[HTML]{363A3D}46.2} & {\color[HTML]{363A3D}57.2} & {\color[HTML]{363A3D}28.1} & {\color[HTML]{363A3D}27.7} & 48.1 \\
% & Pseudocal   & {\color[HTML]{363A3D}10.4} & {\color[HTML]{363A3D}7.3}  & {\color[HTML]{363A3D}4.7}  & {\color[HTML]{363A3D}5.4}  & {\color[HTML]{363A3D}4.4}  & {\color[HTML]{363A3D}14.9} & {\color[HTML]{363A3D}7.4}  & {\color[HTML]{363A3D}4.1}  & {\color[HTML]{363A3D}6.5}  & {\color[HTML]{363A3D}4.4}  & {\color[HTML]{363A3D}25.6} & {\color[HTML]{363A3D}25.5} & 10.0 \\
% & SICL (Ours) & {\color[HTML]{363A3D}9.3}  & {\color[HTML]{363A3D}1.4}  & {\color[HTML]{363A3D}3.6}  & {\color[HTML]{363A3D}1.8}  & {\color[HTML]{363A3D}3.6}  & {\color[HTML]{363A3D}9.8}  & {\color[HTML]{363A3D}3.2}  & {\color[HTML]{363A3D}4.4}  & {\color[HTML]{363A3D}3.3}  & {\color[HTML]{363A3D}9.6}  & {\color[HTML]{363A3D}7.8}  & {\color[HTML]{363A3D}7.4}  & 5.4  \\
% & Acc         & 77.2                    & 68.3                    & 77.6                    & 67.9                    & 77.6                    & 74.3                    & 69.9                    & 78.3                    & 69.8                    & 78.3                    & 56.8                    & 56.4                    &      \\
% \midrule

% \multirow{6}{*}{\textbf{CIFAR-100}}
% & Vanilla TS  & 51.7 & 73.8 & 46.6 & 53.8 & 48.3 & 60.5 & 86.2 & 45.2 & 53.0 & 47.1 & 9.3  & 7.8  & 48.6 \\
% & MC Dropout  & 11.1 & 43.8 & 9.5  & 16.3 & 10.0 & 18.3 & 61.6 & 6.6  & 10.4 & 6.8  & 8.7  & 9.1  & 17.7 \\
% & TransCal    & 43.6 & 17.7 & 48.4 & 29.8 & 46.4 & 33.4 & 8.3  & 50.0 & 32.1 & 47.8 & 23.3 & 22.7 & 33.6 \\
% & Pseudocal   & 6.5  & 30.6 & 10.8 & 6.2  & 6.0  & 12.3 & 32.1 & 5.5  & 6.8  & 5.7  & 31.0 & 31.6 & 15.4 \\
% & SICL (Ours) & 9.7  & 5.5  & 6.0  & 2.5  & 10.1 & 8.9  & 5.6  & 6.1  & 2.4  & 6.0  & 4.5  & 4.7  & 6.0  \\
% & Acc         & 45.7 & 20.9 & 50.6 & 36.7 & 48.6 & 36.9 & 11.2 & 52.2 & 38.8 & 50.0 & 28.3 & 27.6 &      \\
% \midrule

% \multirow{6}{*}{\textbf{ImageNet-C}}
% & Vanilla TS  & 23.9 & 23.2 & 13.4 & 13.4 & 13.2 & 20.7 & 36.4 & 15.7 & 13.7 & 15.7 & 19.8 & 11.9 & 18.4 \\
% & MC Dropout  & 12.1 & 8.6  & 6.8  & 9.2  & 6.7  & 17.9 & 28.0 & 4.1  & 18.4 & 7.9  & 28.9 & 28.8 & 14.8 \\
% & TransCal    & 14.5 & 8.6  & 8.1  & 9.2  & 8.0  & 11.0 & 34.3 & 9.2  & 10.6 & 9.1  & 40.5 & 41.8 & 17.1 \\
% & Pseudocal   & 10.7 & 14.8 & 15.0 & 13.5 & 14.9 & 11.5 & 23.2 & 7.2  & 7.0  & 7.1  & 13.5 & 1.0  & 11.6 \\
% & SICL (Ours) & 16.6 & 2.9  & 3.3  & 2.1  & 3.3  & 8.7  & 3.4  & 2.1  & 0.9  & 1.9  & 10.1 & 8.0  & 5.3  \\
% & Acc         & 2.2  & 7.8  & 7.9  & 7.8  & 7.9  & 2.1  & 8.4  & 8.4  & 8.5  & 8.4  & 44.1 & 45.2 &      \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

\begin{table*}[t]
\centering
\caption{Mean absolute error (MAE) (\%) of the accuracy estimation across various models (ResNet-50, ResNet-101, ViT).}
\label{tab:styled_table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Method}} 
& \multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ResNet-50}} 
& \multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ResNet-101}} 
& \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ViT}} 
& \multicolumn{1}{c}{} \\
\cmidrule(lr){3-7}\cmidrule(lr){8-12}\cmidrule(lr){13-14}
& 
& \cellcolor[HTML]{EFEFEF}\textbf{TENT} 
& \cellcolor[HTML]{EFEFEF}\textbf{EATA} 
& \cellcolor[HTML]{EFEFEF}\textbf{SAR} 
& \cellcolor[HTML]{EFEFEF}\textbf{ROTTA} 
& \cellcolor[HTML]{EFEFEF}\textbf{SOTTA} 
& \cellcolor[HTML]{EFEFEF}\textbf{TENT} 
& \cellcolor[HTML]{EFEFEF}\textbf{EATA} 
& \cellcolor[HTML]{EFEFEF}\textbf{SAR} 
& \cellcolor[HTML]{EFEFEF}\textbf{ROTTA} 
& \cellcolor[HTML]{EFEFEF}\textbf{SOTTA} 
& \cellcolor[HTML]{EFEFEF}\textbf{TENT} 
& \cellcolor[HTML]{EFEFEF}\textbf{SAR} 
& \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}} \\
\midrule

\multirow{7}{*}{\textbf{CIFAR-10}} 
& Vanilla TS  & 12.9 & 17.6 & 23.7 & 21.3 & 23.6 & 11.4 & 18.5 & 23.7 & 21.6 & 23.7 & 11.2 & 10.1 & 18.3 \\
& MC Dropout  & 15.4 & 19.5 & 10.4 & 15.9 & 10.4 & 17.8 & 18.8 & 10.4 & 14.3 & 10.4 & 23.8 & 24.0 & 15.9 \\
& TransCal    & 56.4 & 46.2 & 57.0 & 43.8 & 56.9 & 53.1 & 47.3 & 57.2 & 46.2 & 57.2 & 28.1 & 27.7 & 48.1 \\
& Pseudocal   & 10.4 & 7.3  & 4.7  & 5.4  & 4.4  & 14.9 & 7.4  & 4.1  & 6.5  & 4.4  & 25.6 & 25.5 & 10.0 \\
& SICL (Ours) & 9.3  & 1.4  & 3.6  & 1.8  & 3.6  & 9.8  & 3.2  & 4.4  & 3.3  & 9.6  & 7.8  & 7.4  & 5.4  \\
\cmidrule(lr){2-15}
& Acc         & 77.2 & 68.3 & 77.6 & 67.9 & 77.6 & 74.3 & 69.9 & 78.3 & 69.8 & 78.3 & 56.8 & 56.4 &      \\
\midrule

\multirow{7}{*}{\textbf{CIFAR-100}}
& Vanilla TS  & 51.7 & 73.8 & 46.6 & 53.8 & 48.3 & 60.5 & 86.2 & 45.2 & 53.0 & 47.1 & 9.3  & 7.8  & 48.6 \\
& MC Dropout  & 11.1 & 43.8 & 9.5  & 16.3 & 10.0 & 18.3 & 61.6 & 6.6  & 10.4 & 6.8  & 8.7  & 9.1  & 17.7 \\
& TransCal    & 43.6 & 17.7 & 48.4 & 29.8 & 46.4 & 33.4 & 8.3  & 50.0 & 32.1 & 47.8 & 23.3 & 22.7 & 33.6 \\
& Pseudocal   & 6.5  & 30.6 & 10.8 & 6.2  & 6.0  & 12.3 & 32.1 & 5.5  & 6.8  & 5.7  & 31.0 & 31.6 & 15.4 \\
& SICL (Ours) & 9.7  & 5.5  & 6.0  & 2.5  & 10.1 & 8.9  & 5.6  & 6.1  & 2.4  & 6.0  & 4.5  & 4.7  & 6.0  \\
\cmidrule(lr){2-15}
& Acc         & 45.7 & 20.9 & 50.6 & 36.7 & 48.6 & 36.9 & 11.2 & 52.2 & 38.8 & 50.0 & 28.3 & 27.6 &      \\
\midrule

\multirow{7}{*}{\textbf{ImageNet-C}}
& Vanilla TS  & 23.9 & 23.2 & 13.4 & 13.4 & 13.2 & 20.7 & 36.4 & 15.7 & 13.7 & 15.7 & 19.8 & 11.9 & 18.4 \\
& MC Dropout  & 12.1 & 8.6  & 6.8  & 9.2  & 6.7  & 17.9 & 28.0 & 4.1  & 18.4 & 7.9  & 28.9 & 28.8 & 14.8 \\
& TransCal    & 14.5 & 8.6  & 8.1  & 9.2  & 8.0  & 11.0 & 34.3 & 9.2  & 10.6 & 9.1  & 40.5 & 41.8 & 17.1 \\
& Pseudocal   & 10.7 & 14.8 & 15.0 & 13.5 & 14.9 & 11.5 & 23.2 & 7.2  & 7.0  & 7.1  & 13.5 & 1.0  & 11.6 \\
& SICL (Ours) & 16.6 & 2.9  & 3.3  & 2.1  & 3.3  & 8.7  & 3.4  & 2.1  & 0.9  & 1.9  & 10.1 & 8.0  & 5.3  \\
\cmidrule(lr){2-15}
& Acc         & 2.2  & 7.8  & 7.9  & 7.8  & 7.9  & 2.1  & 8.4  & 8.4  & 8.5  & 8.4  & 44.1 & 45.2 &      \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/main_table.tex <==

% \definecolor{verylightgreen}{#E2FFE1}
\begin{table*}[t]
\centering
\caption{Expected Calibration Error (ECE) (\%) of uncertainty estimation on CIFAR10-C, CIFAR100-C, and ImageNet-C across five TTA methods under benign and dynamic test streams. \textbf{Bold} numbers represent the lowest error.}
\label{tab:main_results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllccccccccccccc} % 3+5+5+2+1 = 16 columns
\toprule
\multicolumn{1}{c}{\textbf{Stream}} & \multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Method}} 
& \multicolumn{5}{c}{\textbf{ResNet-50}} 
& \multicolumn{5}{c}{\textbf{ResNet-101}} 
& \multicolumn{2}{c}{\textbf{ViT}} 
& \multicolumn{1}{c}{\textbf{Avg.}}\\
\cmidrule(lr){4-8}\cmidrule(lr){9-13}\cmidrule(lr){14-15}  
& & & \textbf{TENT} 
& \textbf{EATA} 
& \textbf{SAR} 
& \textbf{RoTTA} 
& \textbf{SoTTA} 
& \textbf{TENT} 
& \textbf{EATA} 
& \textbf{SAR} 
& \textbf{RoTTA} 
& \textbf{SoTTA} 
& \textbf{TENT} 
& \textbf{SAR} 
& \multicolumn{1}{c}{} 
\\
\midrule
\multirow{18}{*}{\textbf{Benign}} 
  & \multirow{6}{*}{\textbf{CIFAR10-C}} 
    & Vanilla TS  & 22.7 & 22.3 & 22.2 & 22.9 & 22.8 & 32.0 & 21.2 & 21.8 & 21.7 & 21.8 & 17.2 & 15.2 & {21.9} \\
  & 
    & MC Dropout  & 16.3 & 11.1 & 10.2 & 10.0 & 10.4 & 25.9 & 10.2 & 10.1 & 9.2  & 10.2 & 22.1 & 19.3 & 13.8 \\
  & 
    & TransCal    & 56.7 & 56.2 & 56.9 & 11.0 & 56.1 & 48.0 & 57.0 & 57.0 & 52.0 & 56.9 & 26.7 & 26.5 & 44.8 \\
  & 
    & PseudoCal   & 9.4  & 7.8  & \textbf{5.2}  & 7.9  & 8.4  & 18.4  & 7.9  & \textbf{5.4}  & 9.0  & 8.6  & 34.9  & 33.6 & 13.9 \\
  & 
    & \cellcolor{verylightblue}\textbf{SICL (Ours)} 
                  & \cellcolor{verylightblue}\textbf{6.4}  
                  & \cellcolor{verylightblue}\textbf{6.9}  
                  & \cellcolor{verylightblue}7.5  
                  & \cellcolor{verylightblue}\textbf{7.1}  
                  & \cellcolor{verylightblue}\textbf{7.5}  
                  & \cellcolor{verylightblue}\textbf{6.6}  
                  & \cellcolor{verylightblue}\textbf{7.6}  
                  & \cellcolor{verylightblue}8.0  
                  & \cellcolor{verylightblue}\textbf{7.3}  
                  & \cellcolor{verylightblue}\textbf{8.0}  
                  & \cellcolor{verylightblue}\textbf{8.4}  
                  & \cellcolor{verylightblue}\textbf{8.7}  
                  & \cellcolor{verylightblue}\textbf{7.7} \\
\cmidrule(lr){3-16}
  & 
    & Acc         & 77.1 & 75.7 & 77.5 & 74.9 & 77.0 & 68.4 & 76.8 & 78.2 & 76.3 & 78.2 & 53.0 & 53.0 &  \\
\cmidrule(lr){2-16}
  & \multirow{6}{*}{\textbf{CIFAR100-C}} 
    & Vanilla TS  & 9.6  & 22.7 & 7.0  & 12.5 & 6.0  & 13.8 & 36.4 & 9.3  & 9.6  & 7.9  & 18.2 & 17.2 & 13.8 \\
  & 
    & MC Dropout  & 13.5 & 16.0 & 8.7  & 13.6 & 8.4  & 20.0 & 12.7 & 9.2  & 8.6  & 8.5  & 19.9 & 18.2 & 12.8 \\
  & 
    & TransCal    & 50.0 & 27.5 & 8.1  & 36.6 & 12.0 & 18.7 & 13.2 & 56.3 & 11.7 & 23.8 & 23.0 & 22.5 & 22.6 \\
  & 
    & PseudoCal   & \textbf{7.4} & 7.3  & 8.7  & 8.1  & 9.0  & 10.8 & 7.4  & \textbf{8.4} & 7.5  & 6.6  & 34.9 & 33.6 & 13.5 \\
  & 
    & \cellcolor{verylightblue}\textbf{SICL (Ours)} 
                  & \cellcolor{verylightblue}7.5  
                  & \cellcolor{verylightblue}\textbf{6.6}  
                  & \cellcolor{verylightblue}\textbf{7.9}  
                  & \cellcolor{verylightblue}\textbf{6.2}  
                  & \cellcolor{verylightblue}\textbf{7.7}  
                  & \cellcolor{verylightblue}\textbf{5.4}  
                  & \cellcolor{verylightblue}\textbf{5.6}  
                  & \cellcolor{verylightblue}6.6  
                  & \cellcolor{verylightblue}\textbf{5.3}  
                  & \cellcolor{verylightblue}\textbf{6.6}  
                  & \cellcolor{verylightblue}\textbf{8.4}  
                  & \cellcolor{verylightblue}\textbf{8.7}  
                  & \cellcolor{verylightblue}\textbf{6.8} \\
\cmidrule(lr){3-16}
  & 
    & Acc         & 52.7 & 33.1 & 54.2 & 49.7 & 51.1 & 44.1 & 19.4 & 55.8 & 51.6 & 52.5 & 50.8 & 50.9 &  \\
\cmidrule(lr){2-16}
  & \multirow{6}{*}{\textbf{ImageNet-C}} 
    & Vanilla TS  & 23.9 & 23.2 & 13.4 & 13.4 & 13.2 & 20.7 & 36.4 & 15.7 & 13.7 & 15.7 & 19.8 & 11.9 & 17.4 \\
  & 
    & MC Dropout  & 11.0 & 13.7 & 15.2 & 14.6 & 16.8 & 12.0 & 12.7 & 13.6 & 11.8 & 12.6 & 28.9 & 28.8 & 16.7 \\
  & 
    & TransCal    & 14.5 & 8.6  & \textbf{8.1}  & 9.2  & 9.8  & \textbf{11.0} & 34.3 & 19.2 & 10.6 & 11.1 & 40.5 & 41.8 & 19.6 \\
  & 
    & PseudoCal   & 14.1 & 8.5  & 14.9 & 13.7 & 14.9 & 14.0 & 11.6 & 14.7 & 12.9 & 14.8 & 19.0 & 17.4 & 14.8 \\
  & 
    & \cellcolor{verylightblue}\textbf{SICL (Ours)} 
                  & \cellcolor{verylightblue}\textbf{10.0}  
                  & \cellcolor{verylightblue}\textbf{7.4}  
                  & \cellcolor{verylightblue}9.1  
                  & \cellcolor{verylightblue}\textbf{7.2}  
                  & \cellcolor{verylightblue}\textbf{8.4}  
                  & \cellcolor{verylightblue}13.6  
                  & \cellcolor{verylightblue}\textbf{9.6}  
                  & \cellcolor{verylightblue}\textbf{12.4}  
                  & \cellcolor{verylightblue}\textbf{9.2}  
                  & \cellcolor{verylightblue}\textbf{10.9}  
                  & \cellcolor{verylightblue}\textbf{15.5}  
                  & \cellcolor{verylightblue}\textbf{11.1}  
                  & \cellcolor{verylightblue}\textbf{10.7} \\
\cmidrule(lr){3-16}
  & 
    & Acc         & 36.3 & 21.0 & 33.2 & 31.1 & 29.0 & 40.0 & 22.9 & 36.3 & 32.7 & 30.5 & 40.7 & 49.0 &  \\
\midrule
\multirow{18}{*}{\textbf{Dynamic}} & \multirow{7}{*}{\textbf{CIFAR10-C}}
& Vanilla TS  & 12.9 & 18.4 & 23.7 & 21.3 & 23.6 & 11.4 & 18.5 & 23.7 & 21.6 & 23.7 & 11.2 & 10.1 & 18.3 \\
&  & MC Dropout  & 15.4 & 18.7 & 10.4 & 15.9 & 10.4 & 17.8 & 19.5 & 10.4 & 14.3 & 10.4 & 23.8 & 24.0 & 15.9 \\
&  & TransCal    & 56.4 & 47.3 & 57.0 & 43.8 & 56.9 & 53.1 & 46.2 & 57.2 & 46.2 & 57.2 & 28.1 & 27.7 & 48.1 \\
&  & PseudoCal   & 17.1 & 7.5  & 12.4 & 14.1 & 12.5 & 23.4 & 7.3 & 12.5 & 14.4 & 12.5 & 25.6 & 25.5 & 15.4 \\
&  & \cellcolor{verylightblue}\textbf{SICL (Ours)} & \cellcolor{verylightblue}\textbf{5.9}  & \cellcolor{verylightblue}\textbf{5.8}  & \cellcolor{verylightblue}\textbf{6.9}  &\cellcolor{verylightblue} \textbf{6.2}  & \cellcolor{verylightblue}\textbf{6.9}  & \cellcolor{verylightblue}\textbf{6.6}  & \cellcolor{verylightblue}\textbf{6.3}  & \cellcolor{verylightblue}\textbf{7.3}  & \cellcolor{verylightblue}\textbf{7.1}  & \cellcolor{verylightblue}\textbf{7.4}  & \cellcolor{verylightblue}\textbf{7.8}  & \cellcolor{verylightblue}\textbf{7.4}  & \cellcolor{verylightblue}\textbf{7.1}  \\
\cmidrule(lr){3-16}
&  & Acc & 77.2 & 68.6 & 77.6 & 67.9 & 77.6 & 74.3 & 70.2 & 78.3 & 69.8 & 78.3 & 56.8 & 56.4 &  \\\cmidrule(lr){2-16}
%\midrule

& \multirow{7}{*}{\textbf{CIFAR100-C}}
& Vanilla TS  & 51.7 & 55.3 & 46.6 & 53.8 & 48.3 & 60.5 & 54.4 & 45.2 & 53.0 & 47.1 & 9.3  & 7.8  & 44.4 \\
& & MC Dropout  & 11.1 & 19.4 & 9.5  & 16.3 & 10.0 & 18.3 & 22.3 & 6.6  & 10.4 & 6.8  & 8.7  & 9.1  & 12.4 \\
&  & TransCal    & 43.6 & 34.5 & 48.4 & 29.8 & 46.4 & 33.4 & 35.9 & 50.0 & 32.1 & 47.8 & 23.3 & 22.7 & 37.3 \\
&  & PseudoCal   & 21.2 & 9.7  & 16.3 & 19.4 & 16.3 & 30.6 & 8.9 & 15.8 & 18.2 & 15.0 & 31.0 & 31.6 & 19.5 \\
&  & \cellcolor{verylightblue}\textbf{SICL (Ours)} & \cellcolor{verylightblue}\textbf{6.6}  & \cellcolor{verylightblue}\textbf{4.4}  & \cellcolor{verylightblue}\textbf{7.8}  & \cellcolor{verylightblue}\textbf{3.8}  & \cellcolor{verylightblue}\textbf{8.0}  & \cellcolor{verylightblue}\textbf{4.6}  & \cellcolor{verylightblue}\textbf{4.5}  & \cellcolor{verylightblue}\textbf{6.6}  & \cellcolor{verylightblue}\textbf{3.5}  & \cellcolor{verylightblue}\textbf{6.5}  & \cellcolor{verylightblue}\textbf{4.5}  & \cellcolor{verylightblue}\textbf{4.7}  & \cellcolor{verylightblue}\textbf{5.5}  \\
\cmidrule(lr){3-16}
&  & Acc & 45.7 & 43.7 & 50.6 & 36.7 & 48.6 & 36.9 & 44.7 & 52.2 & 38.8 & 50.0 & 28.3 & 27.6 &  \\\cmidrule(lr){2-16}
%\midrule

& \multirow{7}{*}{\textbf{ImageNet-C}}
& Vanilla TS  & 23.9 & 14.2 & 13.4 & 13.4 & 13.2 & 20.7 & 9.5 & 15.7 & 13.7 & 15.7 & 19.8 & 11.9 & 15.4 \\
&  & MC Dropout  & 12.1 & 12.4 & 6.8  & 9.2 & 6.7  & 17.9 & 15.9  & 14.1  & 18.4  & 7.9  & 28.9 & 28.8 & 14.9 \\
&  & TransCal    & 14.5 & 29.5 & \textbf{8.1}  & 9.2  & 8.0  & \textbf{11.0} & 32.2 & 9.2  & 10.6 & 9.1  & 40.5 & 41.8 & 18.6 \\
&  & PseudoCal   & 10.7 & 8.1 & 15.0  & 13.5  & 14.9  & 11.5 & 8.7  & \textbf{7.2}  & 9.0 & 7.1  & 13.5  & 11.0  & 10.9 \\
&  & \cellcolor{verylightblue}\textbf{SICL (Ours)} & \cellcolor{verylightblue}\textbf{8.9}  & \cellcolor{verylightblue}\textbf{7.7}  & \cellcolor{verylightblue}8.7  & \cellcolor{verylightblue}\textbf{6.5}  & \cellcolor{verylightblue}\textbf{6.3}  & \cellcolor{verylightblue}12.4  & \cellcolor{verylightblue}\textbf{8.5}  & \cellcolor{verylightblue}8.3  & \cellcolor{verylightblue}\textbf{8.4}  & \cellcolor{verylightblue}\textbf{6.9}  & \cellcolor{verylightblue}\textbf{10.1}  & \cellcolor{verylightblue}\textbf{8.0}  & \cellcolor{verylightblue}\textbf{8.4}  \\
\cmidrule(lr){3-16}
&  & Acc & 37.5 & 31.9 & 36.7 & 34.1 & 31.2 & 33.8 & 34.0 & 32.4 & 31.6 & 33.2 & 44.1 & 45.2 &  \\
%\bottomrule
\bottomrule
\end{tabular}%
}
\end{table*}


% \begin{table*}[t]
% \centering
% \caption{Expected Calibration Error (ECE) (\%) of uncertainty estimation on CIFAR-10C, CIFAR-100C, and ImageNet-C across five TTA methods under dynamic test streams. \textbf{Bold} numbers represent the lowest error.}
% \label{tab:main_results_dynamic}
% \resizebox{.9\textwidth}{!}{%
% \begin{tabular}{llccccccccccccc}
% \toprule
% \multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Method}} 
% & \multicolumn{5}{c}{\textbf{ResNet-50}} 
% & \multicolumn{5}{c}{\textbf{ResNet-101}} 
% & \multicolumn{2}{c}{\textbf{ViT}} 
% & \multicolumn{1}{c}{} \\
% \cmidrule(lr){3-7}\cmidrule(lr){8-12}\cmidrule(lr){13-14}
% & 
% & \textbf{TENT} 
% & \textbf{EATA} 
% & \textbf{SAR} 
% & \textbf{RoTTA} 
% & \textbf{SoTTA} 
% & \textbf{TENT} 
% & \textbf{EATA} 
% & \textbf{SAR} 
% & \textbf{RoTTA} 
% & \textbf{SoTTA} 
% & \textbf{TENT} 
% & \textbf{SAR} 
% & \multicolumn{1}{c}{Avg.} \\
% \midrule

% \multirow{7}{*}{\textbf{CIFAR10-C}}
% & Vanilla TS  & 12.9 & 18.4 & 23.7 & 21.3 & 23.6 & 11.4 & 18.5 & 23.7 & 21.6 & 23.7 & 11.2 & 10.1 & 18.3 \\
% & MC Dropout  & 15.4 & 18.7 & 10.4 & 15.9 & 10.4 & 17.8 & 19.5 & 10.4 & 14.3 & 10.4 & 23.8 & 24.0 & 15.9 \\
% & TransCal    & 56.4 & 47.3 & 57.0 & 43.8 & 56.9 & 53.1 & 46.2 & 57.2 & 46.2 & 57.2 & 28.1 & 27.7 & 48.1 \\
% & PseudoCal   & 17.1 & 7.5  & 12.4 & 14.1 & 12.5 & 23.4 & 7.3 & 12.5 & 14.4 & 12.5 & 25.6 & 25.5 & 15.4 \\
% & \cellcolor{verylightblue}\textbf{SICL (Ours)} & \cellcolor{verylightblue}\textbf{5.9}  & \cellcolor{verylightblue}\textbf{5.8}  & \cellcolor{verylightblue}\textbf{6.9}  &\cellcolor{verylightblue} \textbf{6.2}  & \cellcolor{verylightblue}\textbf{6.9}  & \cellcolor{verylightblue}\textbf{6.6}  & \cellcolor{verylightblue}\textbf{6.3}  & \cellcolor{verylightblue}\textbf{7.3}  & \cellcolor{verylightblue}\textbf{7.1}  & \cellcolor{verylightblue}\textbf{7.4}  & \cellcolor{verylightblue}\textbf{7.8}  & \cellcolor{verylightblue}\textbf{7.4}  & \cellcolor{verylightblue}\textbf{7.1}  \\
% \cmidrule(lr){2-15}
% & Acc & 77.2 & 68.6 & 77.6 & 67.9 & 77.6 & 74.3 & 70.2 & 78.3 & 69.8 & 78.3 & 56.8 & 56.4 &  \\\midrule
% %\midrule

% \multirow{7}{*}{\textbf{CIFAR100-C}}
% & Vanilla TS  & 51.7 & 55.3 & 46.6 & 53.8 & 48.3 & 60.5 & 54.4 & 45.2 & 53.0 & 47.1 & 9.3  & 7.8  & 44.4 \\
% & MC Dropout  & 11.1 & 19.4 & 9.5  & 16.3 & 10.0 & 18.3 & 22.3 & 6.6  & 10.4 & 6.8  & 8.7  & 9.1  & 12.4 \\
% & TransCal    & 43.6 & 34.5 & 48.4 & 29.8 & 46.4 & 33.4 & 35.9 & 50.0 & 32.1 & 47.8 & 23.3 & 22.7 & 37.3 \\
% & PseudoCal   & 21.2 & 9.7  & 16.3 & 19.4 & 16.3 & 30.6 & 8.9 & 15.8 & 18.2 & 15.0 & 31.0 & 31.6 & 19.5 \\
% & \cellcolor{verylightblue}\textbf{SICL (Ours)} & \cellcolor{verylightblue}\textbf{6.6}  & \cellcolor{verylightblue}\textbf{4.4}  & \cellcolor{verylightblue}\textbf{7.8}  & \cellcolor{verylightblue}\textbf{3.8}  & \cellcolor{verylightblue}\textbf{8.0}  & \cellcolor{verylightblue}\textbf{4.6}  & \cellcolor{verylightblue}\textbf{4.5}  & \cellcolor{verylightblue}\textbf{6.6}  & \cellcolor{verylightblue}\textbf{3.5}  & \cellcolor{verylightblue}\textbf{6.5}  & \cellcolor{verylightblue}\textbf{4.5}  & \cellcolor{verylightblue}\textbf{4.7}  & \cellcolor{verylightblue}\textbf{5.5}  \\
% \cmidrule(lr){2-15}
% & Acc & 45.7 & 43.7 & 50.6 & 36.7 & 48.6 & 36.9 & 44.7 & 52.2 & 38.8 & 50.0 & 28.3 & 27.6 &  \\\midrule
% %\midrule

% \multirow{7}{*}{\textbf{ImageNet-C}}
% & Vanilla TS  & 23.9 & 14.2 & 13.4 & 13.4 & 13.2 & 20.7 & 9.5 & 15.7 & 13.7 & 15.7 & 19.8 & 11.9 & 15.4 \\
% & MC Dropout  & 12.1 & 12.4 & 6.8  & 9.2 & 6.7  & 17.9 & 15.9  & 14.1  & 18.4  & 7.9  & 28.9 & 28.8 & 14.9 \\
% & TransCal    & 14.5 & 29.5 & \textbf{8.1}  & 9.2  & 8.0  & \textbf{11.0} & 32.2 & 9.2  & 10.6 & 9.1  & 40.5 & 41.8 & 18.6 \\
% & PseudoCal   & 10.7 & 8.1 & 15.0  & 13.5  & 14.9  & 11.5 & 8.7  & \textbf{7.2}  & 9.0 & 7.1  & 13.5  & 11.0  & 10.9 \\
% & \cellcolor{verylightblue}\textbf{SICL (Ours)} & \cellcolor{verylightblue}\textbf{8.9}  & \cellcolor{verylightblue}\textbf{7.7}  & \cellcolor{verylightblue}8.7  & \cellcolor{verylightblue}\textbf{6.5}  & \cellcolor{verylightblue}\textbf{6.3}  & \cellcolor{verylightblue}12.4  & \cellcolor{verylightblue}\textbf{8.5}  & \cellcolor{verylightblue}8.3  & \cellcolor{verylightblue}\textbf{8.4}  & \cellcolor{verylightblue}\textbf{6.9}  & \cellcolor{verylightblue}\textbf{10.1}  & \cellcolor{verylightblue}\textbf{8.0}  & \cellcolor{verylightblue}\textbf{8.4}  \\
% \cmidrule(lr){2-15}
% & Acc & 37.5 & 31.9 & 36.7 & 34.1 & 31.2 & 33.8 & 34.0 & 32.4 & 31.6 & 33.2 & 44.1 & 45.2 &  \\\bottomrule
% %\bottomrule
% \end{tabular}%
% }
% \end{table*}

==> wacv-2026-author-kit-template/figs/analysis.tex <==
\begin{figure}[htbp]
%\begin{figure*}[H]
    \centering
    \includegraphics[width=\columnwidth]{wacv-2026-author-kit-template/figs/raw_figs/qualitative_analysis.pdf}
    %\includegraphics[width=.9\linewidth]{figs/raw_figs/analysis.png}
    \caption{
    Qualitative analysis for style variants. From left to right, each visualize (a) mean \textit{ContentVariance} over various corruption types, and (b) mean \textit{StyleVariance} over various corruption types. 
    %likelihood of prediction correctness since trained model performs content-driven prediction. 
    %This approach allows SICL to produce reliable confidence estimates by focusing on content-driven predictions that remain stable across diverse, realistic style shifts.
    }
    \label{Fig:analysis}
    \vspace{-10pt}
\end{figure}

==> wacv-2026-author-kit-template/figs/backgrounds.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figs/raw_figs/backgrounds.pdf} % Set to \columnwidth to fit within one column
    \caption{Conceptual demonstration of content-driven predictions with style (\textit{e.g.} texture) and content (\textit{e.g.} shape) differentiation.}
    % caption{Demonstration of content-driven predictions by a trained model with style (\textit{e.g.} texture) and content (\textit{e.g.} shape) differentiation.}
    \label{Fig:backgrounds}
    \vspace{-10pt}
\end{figure}



==> wacv-2026-author-kit-template/figs/main_figure.tex <==
\begin{figure*}[t!]
%\begin{figure*}[H]
    \centering
    \includegraphics[width=.8\linewidth]{figs/raw_figs/main_figure.pdf}
    \caption{
    Detailed illustration of the SICL framework, demonstrating how style invariance is leveraged to estimate correctness likelihood. Given an original sample $\mathbf{x}_i$, SICL generates multiple style-shifted variants as ensemble candidates through feature-level style perturbations. Prediction consistency across these variants is used as a final prediction confidence, where high style-invariance indicates a higher confidence.
    %likelihood of prediction correctness since trained model performs content-driven prediction. 
    %This approach allows SICL to produce reliable confidence estimates by focusing on content-driven predictions that remain stable across diverse, realistic style shifts.
    }
    \label{Fig:main_figure}
    \vspace{-10pt}
\end{figure*}

==> wacv-2026-author-kit-template/figs/motivation.tex <==
\begin{figure}[t!]
%\begin{figure*}[H]
    \centering
    \includegraphics[width=\columnwidth]{wacv-2026-author-kit-template/figs/raw_figs/mot.pdf}
    %\includegraphics[width=.9\linewidth]{figs/raw_figs/analysis.pdf}
    \vspace{-20pt}
    \caption{
    Motivative analysis for desirable ensemble candidates. From left to right, each visualize (a) calibration performance comparison between style and content perturbation, and (b) mean \textit{ContentVariance} of ensemble candidates over various corruption types.
    % Motivative analysis for desirable ensemble candidates. From left to right, each visualize (a) calibration performance comparison between style and content perturbation, and (b) mean $\Delta\mathbf{D}_c(z)$ of ensemble candidates between MC dropout and style-shifted representations over various corruption types.
    %likelihood of prediction correctness since trained model performs content-driven prediction. 
    %This approach allows SICL to produce reliable confidence estimates by focusing on content-driven predictions that remain stable across diverse, realistic style shifts.
    }
    \label{Fig:motivation}
    \vspace{-10pt}
\end{figure}

==> wacv-2026-author-kit-template/figs/overview.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figs/raw_figs/overview.pdf} % Set to \columnwidth to fit within one column
    \caption{Conceptual illustration of SICL's idea. SICL estimates correctness likelihood by assessing style invariance. Consistent predictions across style variants (generated by feature perturbation) (bottom) indicate high confidence in correctness, while low style invariance (top) indicate high uncertainty and lower confidence.}
    \label{Fig:overview}
    \vspace{-10pt}
\end{figure}




% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=.8\columnwidth]{figs/raw_figs/overview.pdf}
%     \caption{
%     Concept of SICL
%     }
%     \label{Fig:overview}
%     \vspace{-10pt}
% \end{figure*}

==> wacv-2026-author-kit-template/preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> wacv-2026-author-kit-template/sec/0_abstract.tex <==
\begin{abstract}


Test-time adaptation (TTA) enables efficient adaptation of deployed models, yet it often leads to poorly calibrated predictive uncertainty—a critical issue in high-stakes domains such as autonomous driving, finance, and healthcare. Existing calibration methods typically assume fixed models or static distributions, which leads to degraded performance under real-world, dynamic test conditions. To address these challenges, we introduce \textbf{S}tyle \textbf{I}nvariance as a \textbf{C}orrectness \textbf{L}ikelihood (SICL), a framework that leverages style-invariance for robust uncertainty estimation. SICL estimates instance-wise correctness likelihood by measuring prediction consistency across style-altered variants, requiring only the model’s forward pass. This makes it a plug-and-play, backpropagation-free calibration module compatible with any TTA method. Comprehensive evaluations across four baselines, five TTA methods, and two realistic scenarios with three model architectures demonstrate that SICL reduces calibration error by an average of 13\%p compared to conventional calibration approaches.
\end{abstract}

==> wacv-2026-author-kit-template/sec/1_intro.tex <==
\section{Introduction}\label{sec:intro}
Deep learning has revolutionized numerous domains, yet the real-world deployment of machine learning models continues to face a critical challenge: performance degradation due to distributional shifts. These shifts occur when deployment conditions deviate from the training environment, including variations in environmental conditions, encounters with unseen objects, or the presence of unexpected noise.

\input{figs/overview}
Test-time adaptation (TTA) has emerged as a promising solution to this challenge, assuming a realistic scenario of model deployment - where a deployed model aims to continuously adapt to unseen distribution using unlabeled test data. Thus, recent advances in TTA~\cite{cotta, rotta, sotta, sar, note, yuan2023robust} have increasingly sought to tackle realistic distribution patterns during model deployment, including temporal correlations~\cite{note} and out-of-distribution (OOD) samples~\cite{sotta}. However, a critical aspect in model deployment — ensuring the reliability of model predictions — remains largely unexplored. Consequently, this limits the applicability of TTA methods in risk-sensitive domains such as autonomous driving~\cite{segu2023darth, li2023test}, and medical application~\cite{he2021autoencoder, yang2022dltta, valanarasu2024fly}.

We observe that prior calibration methods, including \textit{temperature-scaling} approaches~\cite{guo2017calibration, wang2020transferable, hupseudo, park2020calibrated} and \textit{ensembling} approaches~\cite{gal2016dropout, lakshminarayanan2017simple}, assume a fixed model and static test distribution, consequently failing in dynamic regime of TTA. Specifically, we find that during TTA: (1) models exhibit varying calibration patterns when faced with varying test distributions (Section~\ref{sec:difficulty-calibration}), and (2) the self-supervised (\textit{e.g.} entropy-minimization) objective utilized in TTA methods~\cite{sotta, rotta, sar, tent} progressively induces overconfidence, undermining the reliability of predictions (Section~\ref{sec:importance-realistic}). This underscores the necessity for a dynamic calibration approach designed to adapt to these evolving conditions.



In light of these challenges, we propose \textit{Style Invariance as a Correctness Likelihood (SICL)}, a robust calibration framework designed for real-world TTA scenarios. Grounded in the causal assumption~\cite{mitrovic2020representation,von2021self} that predictions should depend solely on content rather than style (Section ~\ref{sec:background}), SICL estimates confidence by measuring the consistency between the original prediction and those obtained from style-shifted variants. By further employing relaxation weights based on the variance of style-induced predictions, SICL ensures a robust, instance-specific calibration across diverse, unseen distributions. Notably, SICL is backpropagation-free, making it easily integrable with various TTA baselines.


We evaluate SICL against state-of-the-art calibration baselines~\cite{guo2017calibration, gal2016dropout, wang2020transferable, hupseudo}, upon three widely used benchmarks, namely CIFAR10-C, CIFAR100-C, and ImageNet-C, across two practical scenarios with three model architecture. Our results suggest that SICL consistently outperforms prior calibration methods by a large margin, showing up to 13\%p reduction  in expected calibration errors (ECE) compared to existing calibration methods under all experimental setups (Section \ref{sec:main_results}). Our extensive qualitative analysis validates the \textit{content-preserving} and \textit{style-varying} characteristics of SICL (Section~\ref{sec:analysis}), while our ablative studies demonstrates the effectiveness of each of our components.

\vspace{+0.05in}
We summarize our contributions as follows.
\vspace{+0.05in}
\begin{itemize}

\item
We shed light on the previously underexplored challenges and importance of uncertainty estimation in TTA scenarios, emphasizing the unique complexities posed by evolving models and distributions at test-time.
%\vspace{-0.05in}
\item  
% We introduce SICL, the first framework to leverage style invariance as a correctness likelihood indicator, and content invariance as a collapse indicator by utilizing feature perturbation to simulate diverse realistic shift (\textit{i.e.,} style-variant, content-preserving).
We introduce SICL, the first framework to leverage style invariance for model calibration, demonstrating robust performance under diverse realistic shifts without usage of both source data and target labels.
% and content invariance as a collapse indicator by utilizing feature perturbation to simulate diverse realistic shift (\textit{i.e.,} style-variant, content-preserving).
%\vspace{-0.05in}
\item 
Our method achieves state-of-the-art calibration performance with a large margin across real-world scenarios including dynamic distribution shifts while being seamlessly applicable to various TTA methods.

\end{itemize}


==> wacv-2026-author-kit-template/sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> wacv-2026-author-kit-template/sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> wacv-2026-author-kit-template/sec/7_limitation.tex <==
\section{Limitation}\label{sec:limitation}

SICL has the following limitations. First, it assumes that the online model can perform content-driven predictions. This assumption limits its performance on collapsed model. Although calibration on a collapsed model is impractical, and other calibration methods also face the same challenges, SICL addresses this issue by introducing a relaxation term to reduce overconfidence when collapse occurs.
Second, SICL requires multiple forward passes to generate style variants, a common limitation in ensemble-based methods like MC Dropout. However, SICL don't require multiple forward passes on the whole layer, and it also eliminates the need for memory-intensive backward passes.
Despite these limitations, SICL presents fewer constraints compared to other calibration methods, as shown in Table \ref{tab:calibration_comparison}. Moreover, its ability to produce accurate uncertainty estimates across various test streams regardless of adaptation methods makes it an appealing solution for practitioners.

% Moreoveravoiding additional training and backward passes, which would otherwise consume more memory and computation.



%However, unlike MC Dropout, SICL reduces computational demand by only requiring multiple passes on lower layers. Furthermore, it doesn't require any 

% SICL has the following limitations. First, it assumes that the online model can perform content-driven predictions. This assumption limits SICL’s performance on models that have already collapsed, as it relies on the model’s ability to retain content recognition. Although calibration on a malfuctioned model is impractical, and most methods face challenges in such cases, SICL partially addresses this issue by applying a relaxation weight to reduce overconfidence when collapse occurs.
% Second, SICL requires multiple forward passes to generate style variants for measuring prediction consistency, a common limitation in stochastic methods like MC Dropout. However, SICL offers the advantage of not requiring multiple forward passes on the full model, unlike MC Dropout, and it also eliminates the need for memory-intensive backward passes, which are more demanding than forward passes.

% Despite these limitations, SICL presents fewer constraints compared to other calibration methods, as shown in Table \ref{tab:calibration_comparison}. Moreover, its ability to effectively provide robust uncertainty estimates across various test streams in a method-agnostic manner makes it an appealing choice for practitioners.

==> wacv-2026-author-kit-template/tables/full_table.tex <==
% \begin{table*}[t]
% \centering
% \caption{Mean absolute error (MAE) (\%) of the accuracy estimation across various models (ResNet-50, ResNet-101, ViT).}
% \label{tab:styled_table}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llrrrrrrrrrrrrr}
% \toprule
% \multicolumn{2}{c}{} 
% & \multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ResNet-50}} 
% & \multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ResNet-101}} 
% & \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ViT}} 
% & \multicolumn{1}{c}{} \\
% \cmidrule(lr){3-7}\cmidrule(lr){8-12}\cmidrule(lr){13-14}
% \multicolumn{2}{c}{} 
% & \cellcolor[HTML]{EFEFEF}\textbf{TENT} 
% & \cellcolor[HTML]{EFEFEF}\textbf{EATA} 
% & \cellcolor[HTML]{EFEFEF}\textbf{SAR} 
% & \cellcolor[HTML]{EFEFEF}\textbf{ROTTA} 
% & \cellcolor[HTML]{EFEFEF}\textbf{SOTTA} 
% & \cellcolor[HTML]{EFEFEF}\textbf{TENT} 
% & \cellcolor[HTML]{EFEFEF}\textbf{EATA} 
% & \cellcolor[HTML]{EFEFEF}\textbf{SAR} 
% & \cellcolor[HTML]{EFEFEF}\textbf{ROTTA} 
% & \cellcolor[HTML]{EFEFEF}\textbf{SOTTA} 
% & \cellcolor[HTML]{EFEFEF}\textbf{TENT} 
% & \cellcolor[HTML]{EFEFEF}\textbf{SAR} 
% & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}} \\
% \midrule

% \multirow{6}{*}{\textbf{CIFAR-10}} 
% & Vanilla TS  & {\color[HTML]{363A3D}12.9} & {\color[HTML]{363A3D}17.6} & {\color[HTML]{363A3D}23.7} & {\color[HTML]{363A3D}21.3} & {\color[HTML]{363A3D}23.6} & {\color[HTML]{363A3D}11.4} & {\color[HTML]{363A3D}18.5} & {\color[HTML]{363A3D}23.7} & {\color[HTML]{363A3D}21.6} & {\color[HTML]{363A3D}23.7} & {\color[HTML]{363A3D}11.2} & {\color[HTML]{363A3D}10.1} & 18.3 \\
% & MC Dropout  & {\color[HTML]{363A3D}15.4} & {\color[HTML]{363A3D}19.5} & {\color[HTML]{363A3D}10.4} & {\color[HTML]{363A3D}15.9} & {\color[HTML]{363A3D}10.4} & {\color[HTML]{363A3D}17.8} & {\color[HTML]{363A3D}18.8} & {\color[HTML]{363A3D}10.4} & {\color[HTML]{363A3D}14.3} & {\color[HTML]{363A3D}10.4} & {\color[HTML]{363A3D}23.8} & {\color[HTML]{363A3D}24.0} & 15.9 \\
% & TransCal    & {\color[HTML]{363A3D}56.4} & {\color[HTML]{363A3D}46.2} & {\color[HTML]{363A3D}57.0} & {\color[HTML]{363A3D}43.8} & {\color[HTML]{363A3D}56.9} & {\color[HTML]{363A3D}53.1} & {\color[HTML]{363A3D}47.3} & {\color[HTML]{363A3D}57.2} & {\color[HTML]{363A3D}46.2} & {\color[HTML]{363A3D}57.2} & {\color[HTML]{363A3D}28.1} & {\color[HTML]{363A3D}27.7} & 48.1 \\
% & Pseudocal   & {\color[HTML]{363A3D}10.4} & {\color[HTML]{363A3D}7.3}  & {\color[HTML]{363A3D}4.7}  & {\color[HTML]{363A3D}5.4}  & {\color[HTML]{363A3D}4.4}  & {\color[HTML]{363A3D}14.9} & {\color[HTML]{363A3D}7.4}  & {\color[HTML]{363A3D}4.1}  & {\color[HTML]{363A3D}6.5}  & {\color[HTML]{363A3D}4.4}  & {\color[HTML]{363A3D}25.6} & {\color[HTML]{363A3D}25.5} & 10.0 \\
% & SICL (Ours) & {\color[HTML]{363A3D}9.3}  & {\color[HTML]{363A3D}1.4}  & {\color[HTML]{363A3D}3.6}  & {\color[HTML]{363A3D}1.8}  & {\color[HTML]{363A3D}3.6}  & {\color[HTML]{363A3D}9.8}  & {\color[HTML]{363A3D}3.2}  & {\color[HTML]{363A3D}4.4}  & {\color[HTML]{363A3D}3.3}  & {\color[HTML]{363A3D}9.6}  & {\color[HTML]{363A3D}7.8}  & {\color[HTML]{363A3D}7.4}  & 5.4  \\
% & Acc         & 77.2                    & 68.3                    & 77.6                    & 67.9                    & 77.6                    & 74.3                    & 69.9                    & 78.3                    & 69.8                    & 78.3                    & 56.8                    & 56.4                    &      \\
% \midrule

% \multirow{6}{*}{\textbf{CIFAR-100}}
% & Vanilla TS  & 51.7 & 73.8 & 46.6 & 53.8 & 48.3 & 60.5 & 86.2 & 45.2 & 53.0 & 47.1 & 9.3  & 7.8  & 48.6 \\
% & MC Dropout  & 11.1 & 43.8 & 9.5  & 16.3 & 10.0 & 18.3 & 61.6 & 6.6  & 10.4 & 6.8  & 8.7  & 9.1  & 17.7 \\
% & TransCal    & 43.6 & 17.7 & 48.4 & 29.8 & 46.4 & 33.4 & 8.3  & 50.0 & 32.1 & 47.8 & 23.3 & 22.7 & 33.6 \\
% & Pseudocal   & 6.5  & 30.6 & 10.8 & 6.2  & 6.0  & 12.3 & 32.1 & 5.5  & 6.8  & 5.7  & 31.0 & 31.6 & 15.4 \\
% & SICL (Ours) & 9.7  & 5.5  & 6.0  & 2.5  & 10.1 & 8.9  & 5.6  & 6.1  & 2.4  & 6.0  & 4.5  & 4.7  & 6.0  \\
% & Acc         & 45.7 & 20.9 & 50.6 & 36.7 & 48.6 & 36.9 & 11.2 & 52.2 & 38.8 & 50.0 & 28.3 & 27.6 &      \\
% \midrule

% \multirow{6}{*}{\textbf{ImageNet-C}}
% & Vanilla TS  & 23.9 & 23.2 & 13.4 & 13.4 & 13.2 & 20.7 & 36.4 & 15.7 & 13.7 & 15.7 & 19.8 & 11.9 & 18.4 \\
% & MC Dropout  & 12.1 & 8.6  & 6.8  & 9.2  & 6.7  & 17.9 & 28.0 & 4.1  & 18.4 & 7.9  & 28.9 & 28.8 & 14.8 \\
% & TransCal    & 14.5 & 8.6  & 8.1  & 9.2  & 8.0  & 11.0 & 34.3 & 9.2  & 10.6 & 9.1  & 40.5 & 41.8 & 17.1 \\
% & Pseudocal   & 10.7 & 14.8 & 15.0 & 13.5 & 14.9 & 11.5 & 23.2 & 7.2  & 7.0  & 7.1  & 13.5 & 1.0  & 11.6 \\
% & SICL (Ours) & 16.6 & 2.9  & 3.3  & 2.1  & 3.3  & 8.7  & 3.4  & 2.1  & 0.9  & 1.9  & 10.1 & 8.0  & 5.3  \\
% & Acc         & 2.2  & 7.8  & 7.9  & 7.8  & 7.9  & 2.1  & 8.4  & 8.4  & 8.5  & 8.4  & 44.1 & 45.2 &      \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

\begin{table*}[t]
\centering
\caption{Mean absolute error (MAE) (\%) of the accuracy estimation across various models (ResNet-50, ResNet-101, ViT).}
\label{tab:styled_table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Method}} 
& \multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ResNet-50}} 
& \multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ResNet-101}} 
& \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\textbf{ViT}} 
& \multicolumn{1}{c}{} \\
\cmidrule(lr){3-7}\cmidrule(lr){8-12}\cmidrule(lr){13-14}
& 
& \cellcolor[HTML]{EFEFEF}\textbf{TENT} 
& \cellcolor[HTML]{EFEFEF}\textbf{EATA} 
& \cellcolor[HTML]{EFEFEF}\textbf{SAR} 
& \cellcolor[HTML]{EFEFEF}\textbf{ROTTA} 
& \cellcolor[HTML]{EFEFEF}\textbf{SOTTA} 
& \cellcolor[HTML]{EFEFEF}\textbf{TENT} 
& \cellcolor[HTML]{EFEFEF}\textbf{EATA} 
& \cellcolor[HTML]{EFEFEF}\textbf{SAR} 
& \cellcolor[HTML]{EFEFEF}\textbf{ROTTA} 
& \cellcolor[HTML]{EFEFEF}\textbf{SOTTA} 
& \cellcolor[HTML]{EFEFEF}\textbf{TENT} 
& \cellcolor[HTML]{EFEFEF}\textbf{SAR} 
& \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}} \\
\midrule

\multirow{7}{*}{\textbf{CIFAR-10}} 
& Vanilla TS  & 12.9 & 17.6 & 23.7 & 21.3 & 23.6 & 11.4 & 18.5 & 23.7 & 21.6 & 23.7 & 11.2 & 10.1 & 18.3 \\
& MC Dropout  & 15.4 & 19.5 & 10.4 & 15.9 & 10.4 & 17.8 & 18.8 & 10.4 & 14.3 & 10.4 & 23.8 & 24.0 & 15.9 \\
& TransCal    & 56.4 & 46.2 & 57.0 & 43.8 & 56.9 & 53.1 & 47.3 & 57.2 & 46.2 & 57.2 & 28.1 & 27.7 & 48.1 \\
& Pseudocal   & 10.4 & 7.3  & 4.7  & 5.4  & 4.4  & 14.9 & 7.4  & 4.1  & 6.5  & 4.4  & 25.6 & 25.5 & 10.0 \\
& SICL (Ours) & 9.3  & 1.4  & 3.6  & 1.8  & 3.6  & 9.8  & 3.2  & 4.4  & 3.3  & 9.6  & 7.8  & 7.4  & 5.4  \\
\cmidrule(lr){2-15}
& Acc         & 77.2 & 68.3 & 77.6 & 67.9 & 77.6 & 74.3 & 69.9 & 78.3 & 69.8 & 78.3 & 56.8 & 56.4 &      \\
\midrule

\multirow{7}{*}{\textbf{CIFAR-100}}
& Vanilla TS  & 51.7 & 73.8 & 46.6 & 53.8 & 48.3 & 60.5 & 86.2 & 45.2 & 53.0 & 47.1 & 9.3  & 7.8  & 48.6 \\
& MC Dropout  & 11.1 & 43.8 & 9.5  & 16.3 & 10.0 & 18.3 & 61.6 & 6.6  & 10.4 & 6.8  & 8.7  & 9.1  & 17.7 \\
& TransCal    & 43.6 & 17.7 & 48.4 & 29.8 & 46.4 & 33.4 & 8.3  & 50.0 & 32.1 & 47.8 & 23.3 & 22.7 & 33.6 \\
& Pseudocal   & 6.5  & 30.6 & 10.8 & 6.2  & 6.0  & 12.3 & 32.1 & 5.5  & 6.8  & 5.7  & 31.0 & 31.6 & 15.4 \\
& SICL (Ours) & 9.7  & 5.5  & 6.0  & 2.5  & 10.1 & 8.9  & 5.6  & 6.1  & 2.4  & 6.0  & 4.5  & 4.7  & 6.0  \\
\cmidrule(lr){2-15}
& Acc         & 45.7 & 20.9 & 50.6 & 36.7 & 48.6 & 36.9 & 11.2 & 52.2 & 38.8 & 50.0 & 28.3 & 27.6 &      \\
\midrule

\multirow{7}{*}{\textbf{ImageNet-C}}
& Vanilla TS  & 23.9 & 23.2 & 13.4 & 13.4 & 13.2 & 20.7 & 36.4 & 15.7 & 13.7 & 15.7 & 19.8 & 11.9 & 18.4 \\
& MC Dropout  & 12.1 & 8.6  & 6.8  & 9.2  & 6.7  & 17.9 & 28.0 & 4.1  & 18.4 & 7.9  & 28.9 & 28.8 & 14.8 \\
& TransCal    & 14.5 & 8.6  & 8.1  & 9.2  & 8.0  & 11.0 & 34.3 & 9.2  & 10.6 & 9.1  & 40.5 & 41.8 & 17.1 \\
& Pseudocal   & 10.7 & 14.8 & 15.0 & 13.5 & 14.9 & 11.5 & 23.2 & 7.2  & 7.0  & 7.1  & 13.5 & 1.0  & 11.6 \\
& SICL (Ours) & 16.6 & 2.9  & 3.3  & 2.1  & 3.3  & 8.7  & 3.4  & 2.1  & 0.9  & 1.9  & 10.1 & 8.0  & 5.3  \\
\cmidrule(lr){2-15}
& Acc         & 2.2  & 7.8  & 7.9  & 7.8  & 7.9  & 2.1  & 8.4  & 8.4  & 8.5  & 8.4  & 44.1 & 45.2 &      \\
\bottomrule
\end{tabular}
}
\end{table*}

